Multi-Level Branched Regularization for Federated Learning

A critical challenge of federated learning is data heterogeneity and imbalance across clients, which leads to inconsistency between local networks and unstable convergence of global models. To alleviate the limitations, we propose a novel architectural regularization technique that constructs multiple auxiliary branches in each local model by grafting local and global subnetworks at several different levels and that learns the representations of the main pathway in the local model congruent to the auxiliary hybrid pathways via online knowledge distillation. The proposed technique is effective to robustify the global model even in the non-iid setting and is applicable to various federated learning frameworks conveniently without incurring extra communication costs. We perform comprehensive empirical studies and demonstrate remarkable performance gains in terms of accuracy and efficiency compared to existing methods. The source code is available at our project page.

==> ICML arxiv/algorithms/fedavg.tex <==
% !TEX root = ../main.tex

\iffalse
\begin{algorithm}[t]
\caption{Federated learning framework}
\label{alg:fedavg}
\SetAlgoLined

\KwIn{$\theta^0$, number of clients $N$, number of local iterations $K$, number of communication rounds $T$}
\For{$\text{each round}~t = 0, \dots ,T$}{
Sample subset of clients $S_t \subseteq \{1, \dots, N\}$

Server sends $\theta^t$ to all clients $i \in S_t$ 

\For{$\text{each client}~ i \in S_t,~\textbf{in parallel}$}{
\For{$k = 0, \dots ,K$}{
{$\operatorname*{\underset{\theta_{i,k}^t}{argmin}}\ L_i(\theta_{i,k}^t
)$} ~~~ \dots \cref{fedavg_loss} and \cref{proposed_loss}
}
Client sends  $\theta_{i,K}^t$ back to the server}
\textbf{In server:}

\quad $\theta^{t+1}$ = $\frac{1}{|S_t|} \Sigma_{i \in S_t}\theta_{i,K}^{t}$
}
\textbf{Return} ~ $\theta^{t+1}$ 

\end{algorithm}
\fi

\begin{algorithm}[tb]
   \caption{FedAvg}
   \label{alg:fedavg}
\begin{algorithmic}
   \STATE {\bfseries Input:} {\# of clients $N$, \# of communication rounds $T$, \\ \quad\quad\quad \# of local iterations $K$, initial server model $\theta^0$}
   \FOR{$\text{each}~t = 0, \dots ,T-1$}
   \STATE Sample a subset of clients $S_t \subseteq \{1, \dots, N\}$.
   \STATE Server sends $\theta^t$ to each of the clients $i \in S_t$.
   \FOR{$\text{each client}~ i \in S_t,~\textbf{in parallel}$}
   \STATE \revision{Initialize client model $\theta_{i, 0} = \theta^t$.}
   \FOR{$k = 1, \dots ,K$}
   %\FOR{$\text{each batch } \textbf{b} = \{x,y\} \text{ of } D_i$ }
   \STATE \revision{$q_L \leftarrow \text{softmax} \left (\frac{F_L^M}{\tau} \right)$}
   \STATE \revision{$\mathcal{L}_L \leftarrow \text{CrossEntropy}(q_L, y)$}
   \STATE \revision{$\theta_{i,k}^t \leftarrow \theta_{i,k-1}^t - \eta \nabla \mathcal{L}_L $}
   %\ENDFOR
   %\STATE {\bfseries In server:} \\ \quad $\theta^{t+1}$ = $\frac{1}{|S_t|} \Sigma_{i \in S_t}\theta_{i,K}^{t}$
   \ENDFOR
   \STATE Client sends  $\theta_{i,K}^t$ back to the server.
   \ENDFOR
   \STATE {\bfseries In server:} \\ \quad $\theta^{t+1} = \frac{1}{|S_t|} \sum_{i \in S_t} \theta_{i,K}^{t}$
   \ENDFOR
\end{algorithmic}
\end{algorithm}


==> ICML arxiv/algorithms/proposed_method.tex <==
% !TEX root = ../main.tex
%
%\algnewcommand\algorithmicforeach{\textbf{for each:}}
%\algnewcommand\ForEach{\item[ \algorithmicforeach]}

%\vspace{10pt}
\begin{algorithm}[t]
   \caption{FedMLB}
   \label{alg:proposed_method}
\begin{algorithmic}
   \STATE {\bfseries Input:} {\# of clients $N$, \# of communication rounds $T$, \\ \quad\quad\quad \# of local iterations $K$, initial server model $\theta^0$}
   \FOR{$\text{each round}~t = 1, \dots ,T$}
   \STATE Sample a subset of clients $S_t \subseteq \{1, \dots, N\}$.
   \STATE Server sends $\theta^{t-1}$ to each of all clients $i \in S_t$.
   \FOR{$\text{each}~ i \in S_t,~\textbf{in parallel}$}
   \STATE $\theta_{i,0}^t \leftarrow {\theta^{t-1}}$
   \FOR{$k = {1, \dots ,K}$}
   \FOR {{\bf{each}} $(x,y)$ in a batch}
   %\STATE \revision{}
   \STATE $ q_L(x ; \tau) \leftarrow \text{softmax} \left (\frac{f_L(x; \theta_{i,k-1}^t)}{\tau} \right)$
   \STATE $q_H^m(x ; \tau) \leftarrow \text{softmax} \left (\frac{f_H^m(x ; \theta_{i,m,k-1}^t)}{\tau} \right)$, \\ \quad\quad\quad\quad\quad\ $m = 1, \dots, M-1$
   %\STATE \revision{$\mathcal{L}_L \leftarrow \text{CrossEntropy}(q_L, y)$}
   %\STATE \revision{$\mathcal{L}_{G}^\text{CE} \leftarrow \frac{1}{M-1}\underset{j=1}{\overset{M-1}{\sum}}\text{CrossEntropy}(q_G^j,y)$}
   
   %\STATE \revision{$\mathcal{L}_{G}^{\text{KL}} \leftarrow \frac{1}{M-1}\overset{M-1}{\underset{j=1}{\sum}}\text{KL}(\tilde{q}_G^j,\tilde{q}_L)$}
   \ENDFOR
   \STATE $\mathcal{L}(\theta_{i,k-1}^t) \leftarrow \mathcal{L}_{L} + \lambda_1 \cdot \mathcal{L}_H^{\text{CE}} + \lambda_2 \cdot \mathcal{L}_H^{\text{KL}}$
   \STATE ${\theta_{i,k}^t \leftarrow \theta_{i,k-1}^t - \eta \nabla \mathcal{L} }$  %\ENDFOR
   %\STATE \revision{$\theta_{i,k+1}^t = \operatorname*{\underset{\theta_{i,k}^t}{argmin}}\ L_i(\theta_{i,k}^t)$}
   
   \ENDFOR
   \STATE Client sends  $\theta_{i,K}^t$ back to the server
   \ENDFOR
   \STATE {\bfseries In server:} \\ \quad {$\theta^{t}$ = $\frac{1}{|S_t|} \sum_{i \in S_t}\theta_{i,K}^{t}$}
   \ENDFOR
\end{algorithmic}
\end{algorithm}


==> ICML arxiv/sections/abstract.tex <==
% !TEX root = ../main.tex

%%%%%%%%% ABSTRACT
\begin{abstract}

\iffalse
\revision{
Federated learning is a machine learning setting in which distributed clients collaborate to train a single global model without communication of the raw data with a coordinating server.
However, the heterogeneity in the system and client’s data put many approaches through slow convergence and degraded performance. 
To tackle the problem, we propose a novel federated learning framework, which alleviate the information gaps between global and local models, which is achieved by fusing the multi-level knowledge from global model for local training. 
The proposed algorithm encourages the learned features to preserve global knowledge and have consistent views across local models without additional communication cost. 
We perform comprehensive empirical studies on real data under various settings and demonstrate the remarkable performance of the proposed method in terms of accuracy and communication-efficiency compared to the state-of-the-art methods.}
\fi


%A critical challenge of federated learning is data inconsistency and imbalance across clients, which results in suboptimal convergences of local networks.
A critical challenge of federated learning is data heterogeneity and imbalance across clients, which leads to inconsistency between local networks and unstable convergence of global models.
To alleviate the limitations, we propose a novel architectural regularization technique that constructs multiple auxiliary branches in each local model by grafting local and global subnetworks at several different levels and that learns the representations of the main pathway in the local model congruent to the auxiliary hybrid pathways via online knowledge distillation.
%The auxiliary hybrid pathways learn the representations congruent to the main pathway of the local model, where the parameters in the main pathways are updated with the global network blocks fixed.
%makes the representation of each level in a local model congruent to the global model. 
%Our approach constructs a branch from each level of a local model, where the network structure and the parameters of the branch are borrowed from the global model.
%The goal of the multiple branches is to maintain the representations of local data consistent with the ones of the global one by performing knowledge distillation between the output of the local model and the logits of individual branches.
%Our regularization method is unique in the sense that it does not attempt to preserve model parameters or activations directly while it introduces an additional constraint that aligns the representation of each branch to that of the main pathway.
The proposed technique is effective to robustify the global model even in the non-iid setting and is applicable to various federated learning frameworks conveniently without incurring extra communication costs. 
We perform comprehensive empirical studies and demonstrate remarkable performance gains in terms of accuracy and efficiency compared to existing methods.
The source code is available in our project page\footnote{\url{http://cvlab.snu.ac.kr/research/FedMLB}}.



\iffalse
 Federated learning suffers from difficulties in convergence depending on the heterogeneous data distribution of participating clients. 
 This is because each client can access only the data it has, so the local models trained on local data learn features overfitted to the data of each client.
 To solve this problem, in this report, we propose a method that reduces the loss on local data while simultaneously learning globally meaningful features of the local model.
This is achieved by reducing the loss on local data, and at the same time reducing the loss of logit forwarding intermediate features of the local model to the global model.
As a result of testing on CIFAR 100 and Tiny-ImageNet dataset, the proposed method showed better performance than FedAVG, the baseline of federated learning, and further improved its performance when combined with FedAGM.
\fi
\end{abstract}

==> ICML arxiv/sections/acknowledgments.tex <==
% !TEX root = ../main.tex

\paragraph{Acknowledgments}
\label{Acknowledgments}

%This work was partly supported by Samsung Electronics Co., Ltd., and by the National Research Foundation of Korea (NRF) grant funded by the Korea government (MSIT) (No. 2022R1A2C3012210).

This work was partly supported by Samsung Electronics Co., Ltd., and by the NRF Korea grant [No. 2022R1A2C3012210, Knowledge Composition via Task-Distributed Federated Learning] and the IITP grants [2021-0-02068, Artificial Intelligence Innovation Hub; 2021-0-01343, Artificial Intelligence Graduate School Program (Seoul National University)] funded by the Korea government (MSIT).



==> ICML arxiv/sections/conclusion.tex <==
% !TEX root = ../main.tex

%%%%%%%%% CONCLUSION
%
\section{Conclusion}
\label{sec:conclusion}

We presented a practical solution to improve the performance of federated learning, where a large number of clients with heterogeneous data distributions and limited participation rates are involved in the learning process.
To address the critical limitations, we proposed a novel regularization technique via online knowledge distillation.
Our approach employs multi-level hybrid branched networks, which reduces the drift of the representations in the local models from the feature space of the global model.
The proposed federated learning framework has the following two desirable properties; it requires no additional communication cost and spends no extra memory to store the history of local states.
We demonstrated that the proposed approach, referred to as FedMLB, achieves outstanding performance in terms of accuracy and efficiency, through a comprehensive evaluation on multiple standard benchmarks under various environments.



==> ICML arxiv/sections/experiments.tex <==
% !TEX root = ../main.tex

%%%%%%%%% EXPERIMENTS





%\input{tables/lambdaCE_analysis.tex}
%\input{tables/lambdaKL_analysis.tex}


\section{Experiments}
\label{sec:experiments}

This section demonstrates the effectiveness of FedMLB by incorporating it into various baseline algorithms for federated learning.
%\input{tables/moderate_clients.tex}
%\input{tables/large_clients.tex}




\subsection{Experimental setup}
\paragraph{Datasets and baselines}
%We conduct a set of experiments on the CIFAR-100, and Tiny-ImageNet\footnote{\url{https://www.kaggle.com/c/tiny-imagenet}}~\cite{le2015tiny} datasets.
We conduct a set of experiments on the CIFAR-100 and Tiny-ImageNet~\cite{le2015tiny} datasets.
%For the non-iid data simulation, we sample data with heterogenous label ratios using a Dirichlet distribution with two parameters \{0.3, 0.6\}, following~\cite{hsu2019measuring}.
To simulate non-iid data, we sample examples with heterogeneous label ratios using symmetric Dirichlet distributions parametrized by two different concentration parameters \{0.3, 0.6\}, following~\cite{hsu2019measuring}.
%\jkkim{To simulate non-iid data, we sample examples of each client from a symmetric Dirichlet distribution over labels with concentration parameter  \{0.3, 0.6\}, following ~\cite{hsu2019measuring}.}
%\jkkim{To simulate non-iid data, we draw class prior vectors for each client using Dirichlet distribution with concentration parameter  \{0.3, 0.6\}, following ~\cite{hsu2019measuring}.
%Then 
%Each client's examples are sampled from an associated multinomial distribution over labels.
%The multinomial is drawn from a symmetric Dirichlet distribution }
We maintain the training dataset sizes balanced, so each client holds the same number of examples.
For comprehensive evaluation, we employ several state-of-the-art federated learning techniques including FedAvg~\cite{mcmahan2017communication}, FedAvgM~\cite{hsu2019measuring}, FedADAM~\cite{reddi2021adaptive}, and FedDyn~\cite{acar2020federated}.
We also compare with existing regularization-based approaches such as FedProx~\cite{li2020federated}, FedLS-NTD~\cite{lee2021preservation}, and FedGKD~\cite{yao2021local}.
We choose a ResNet-18~\cite{he2016deep} as the backbone network for all benchmarks, but replace the batch normalization with group normalization as suggested in~\cite{hsieh2020non}.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/Addwithbaseline_5.pdf}
\vspace{-0.6cm}
\caption{The convergence plots of FedMLB and other federated learning baselines on CIFAR-100.
The + symbol indicates the incorporation of FedMLB.
The number of clients, the participation rate, and the symmetric Dirichlet parameter are set to 100,  5\%, and 0.3, respectively.}
\vspace{-0.2cm}
\label{fig:main_convergence_plot_baseline}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/main_convergence_plot_distill.pdf}
\vspace{-0.6cm}
\caption{The convergence plots of FedMLB and other local optimization techniques on CIFAR-100.
%The * symbol shows the results when the method is applied to local objective of FedAvg.
The number of clients, the participation rate, and the symmetric Dirichlet parameter are set to 100,  5\%, and 0.3, respectively.}
\vspace{-0.2cm}
\label{fig:main_convergence_plot_distill}
\end{figure}




%\input{tables/KD_FitNet.tex}
%\input{tables/Feddistill.tex}

\input{tables/local_approaches.tex}
\input{tables/moreiteration.tex}


\input{tables/LFGN.tex}


%\vspace{-0.2cm}
\paragraph{Evaluation metrics}
To evaluate generalization performance of each algorithm, we use the whole test set in the CIFAR-100~\cite{krizhevsky2009learning} and Tiny-ImageNet datasets.
Since both convergence speed as well as final performance are important metrics for federated learning as discussed in~\cite{al2020federated}, we measure the performance attained at two specific rounds and the number of required rounds to achieve the desired levels of the target accuracy.
For the methods that fail to accomplish the target accuracy within the maximum communication rounds, we append a $+$ sign to the number indicating the communication round.





%\vspace{-0.2cm}
\paragraph{Implementation details}

We use PyTorch~\cite{paszke2019pytorch} to implement the proposed method and other baselines.
FedMLB divides its backbone network, ResNet-18, into six blocks based on the depths of its layers and feature map sizes; each of conv1, conv2\_x, conv3\_x, conv4\_x, conv5\_x, and fc layers constitutes a single block.
Following~\cite{acar2020federated, xu2021fedcm}, we adopt the SGD optimizer for local updates with the learning rate of $0.1$ for all benchmarks, except for the FedADAM whose learning rate is set to $0.01$.
We apply the exponential decay to the local learning rate with the parameter of 0.998.
%We apply exponential decay on the local learning rate with a parameter selected from $\{1.0, 0.998, 0.995\}$.
There is no momentum in the local SGD but the weight decay with a factor of 0.001 is employed to prevent overfitting.
We also perform gradient clipping to stabilize the algorithms.
The number of local training epochs is set to 5, and the batch size is determined to make the total number of iterations for local updates $50$ for all experiments unless specified otherwise.
The global learning rate is $1$ for all methods except for FedADAM with $0.01$.
We list the details of the hyperparameters specific to FedMLB and the baseline algorithms in Appendix~\ref{ad:imple_details}.




\subsection{Main results}
\paragraph{FedMLB with server-side optimization techniques}
We first present the performance of the proposed approach, FedMLB, on CIFAR-100 and Tiny-ImageNet based on four federated learning baselines that perform server-side optimizations.
Our experiments have been performed on two different settings; one is with moderate-scale, which involves 100 devices with 5\% participation rate per round, and the other is with a large number of clients, 500 with 2\% participation rate.
Note that the number of clients in the large-scale setting is 5 times more than the moderate-scale experiment, which reduces the number of examples per client by 80\%.
%Specifically, each client has 100 and 200 data points in CIFAR-10 and Tiny-ImageNet, respectively.
Table~\ref{tab:moderate_and_large_scales} demonstrates that FedMLB improves accuracy and convergence speed by significant margins consistently on all the four baselines for most cases.
Figure~\ref{fig:main_convergence_plot_baseline} also illustrates the effectiveness of FedMLB when it is combined with the four baseline methods.
Note that the overall performance in the large-scale setting is lower than the case with a moderate number of clients. 
This is because, as the number of training data per client decreases, each client has even more distinct properties and is prone to drift.
Nevertheless, we observe that FedMLB outperforms the baseline methods consistently on all benchmarks.


\iffalse
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/BranchAnalysis.pdf}
\caption{Performance comparison between the proposed method using multiple auxiliary branches and the model using only one branch. The hybrid pathway index follows the notation in Figure~\ref{fig:framework}.}
\label{fig:branch_analysis}
\end{figure}
\fi
%
\input{tables/hybrid_pathways} 
\input{tables/avgacc_numofbranches} 
%
%\vspace{-0.3cm}
\paragraph{Comparisons with other local objectives}
To understand the effectiveness of FedMLB compared to other local optimization techniques, we compare our objective with the following two baselines: 1) employing the vanilla knowledge distillation for regularization (FedAvg + KD)~\cite{hinton2014distilling}), and 2) adopting knowledge distillation on block-wise features between the local and global model (FedAvg + FitNet~\cite{romero2014fitnets}).  

Table~\ref{tab:local_approaches} illustrates the outstanding performance of our multi-level branched regularization using online knowledge distillation on CIFAR-100, and Figure~\ref{fig:main_convergence_plot_distill} visualizes the convergence curves of all compared algorithms with different local objectives.
One noticeable result is that the baseline methods with knowledge distillation only achieve marginal gains or sometimes degrade accuracy.
This is partly because the predictions of the downloaded global model are not fully-trustworthy during training, especially in early communication rounds.
Therefore, merely simulating the outputs of the global model is suboptimal and hampers the learning process at the local model. 
In this respect, FedMLB is more robust to heterogeneous characteristics of clients and more flexible to learn the new knowledge in local models.
Note that, FedGKD requires 1.5 times communication costs compared to other methods since the server transmits the historical global model along with the latest model for server-to-client communication.



\iffalse
\revision{
Table~\ref{tab:local_approaches}~shows the performance comparison between methods of using the global distribution knowledge of the global model for local learning by modifying the local objective.
The part above the dotted line of the Table~\ref{tab:local_approaches} is the application of the existing knowledge distillation method using the global model as the teacher model. "FedAvg + KD" is a method of minimizing KL divergence of the soft label of the global model and the local model.
"FedAvg + PodNet (FitNet)" is a method of minimizing the layerwise L2 distance of the activation of the global model and the local model.}

\revision{
[The proposed method is knowledge distillation specialized for federated learning setting.]
In the case of centralized learning where data is gathered on one server, the teacher model of knowledge distillation is often a model with more layers and parameters than the study model and with more knowledge about tasks. 
However, this is not the case for the early-stage global model in Federated learning. 
This is because the global model is the initial point of the local model, and while having a good knowledge of global data distribution, there is still much room for improvement in features as an unskilled model. 
Therefore, applying the existing knowledge distillation method directly to federated learning to preserve the byproduct of the global model as it is may have side effects that prevent the local model from learning improved features compared to the global model. 
In this respect, our method is able to effectively bypass this trade-off by not having to mimic the fixed output of the global model, which leads to a noticeable gain compared to other methods in the experimental results.}
\fi



\subsection{Effect of more local iterations}
The increase of local iterations under a heterogeneous environment is beneficial because we can reduce the number of communication rounds between the server and clients.
Table~\ref{tab:abl_local_iterations} presents the results of FedMLB and the baselines with more local iterations, \textit{i.e.}, $K \in \{100, 200\}$, on CIFAR-100.
\iffalse
\revision{We can first observe that while the increasing local iteration shows little or rather no performance gain for baseline methods.
This is because the increase of local iterations is prone to result in trade off between additional optimization procedure and more divergence across client models.
In contrast, the proposed method shows continuous performance gain as the local iteration increases, which implies that the proposed regularization effectively handles client drift issue during local updates toward heterogeneous data.}
\fi
The results demonstrate that FedMLB outperforms the compared methods by significant margins.
An interesting observation is that the baseline methods fail to benefit from additional iterations.
This is because the increase of local iterations is prone to result in more divergence across multiple client models and eventually leads to degradation of performance.
In contrast, FedMLB consistently improves its accuracy and convergence speed substantially compared to the results with 50 iterations shown in Table~\ref{tab:local_approaches}.
Although the accuracies with 100 and 200 iterations are similar, the numbers of required iterations to achieve 40\% and 48\% are noticeably smaller with 200 iterations. 
These results imply that FedMLB handles the client drift issue effectively.


%

\input{tables/lambda_analysis.tex}
\input{tables/temp_analysis.tex}

\iffalse
\begin{figure*}[h]
\centering
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figures/Addwithbaseline_5.pdf}
\caption{Combining FedMLB to federated learning baselines.}
\end{subfigure}
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figures/Feddistill_5.pdf}
\caption{Comparison with regularization-based methods}
\end{subfigure}
\caption{The convergence plot of two experiments on CIFAR-100. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and 0.3, respectively.}
\label{fig:main_convergence_plot}
\end{figure*}
\fi



\subsection{Analysis of auxiliary branches}

%\vspace{-0.2cm}
\paragraph{Effectiveness of local-to-global pathways}

Each hybrid pathway in FedMLB is composed of a set of local blocks followed by a global subnetwork.
To show the effectiveness of the current design of the hybrid pathways, we evaluate the performance of the opposite architecture design, the local model with multi-level global-to-local pathways.
As in the original version of FedMLB, the newly considered model denoted by $\text{FedMLB}_{\text{G} \rightarrow \text{L}}$ also updates the parameters in the local blocks only.
Table~\ref{tab:abl_branch_type} presents that the knowledge distillation with the hybrid pathways stemming from local blocks to global ones outperforms the opposite composition method.
The reason is that $\text{FedMLB}_{\text{G} \rightarrow \text{L}}$ constrains the output of each local blocks excessively and reduces the flexibility of the main pathway in the local network significantly.
Although the new strategy is helpful for preserving the knowledge in the global model, it interferes learning new knowledge. 
%On the other hand, $\text{FedMLB}_{\text{L} \rightarrow \text{G}}$ may mitigate this issue in that it regularizes the newly learned knowledge so that it makes sense globally.

%\vspace{-0.2cm}
\paragraph{Effect of multi-level branches}

FedMLB employs the features from multi-level auxiliary branches to compute the cross-entropy loss $\mathcal{L}_H^{\text{CE}}$ and KL-divergence loss $\mathcal{L}_H^{\text{KL}}$.
\iffalse
Figure~\ref{fig:branch_analysis} illustrates that the use of all auxiliary branches leads to the best performance and the proposed multi-level regularization contributes to additional performance gains.
It also implies that the branches stemming from deeper local blocks are less helpful.
\fi
Table~\ref{tab:path_combinations} illustrates that the pathways grafted from the lower layers are generally more helpful for accuracy gains.
Also, according to Table~\ref{tab:avgacc_numofbranches}, the accuracy of FedMLB generally improves as we increase the number of pathways.
%This result implies that preservation of representations of global model in early layers is crucial for preventing client drift caused by heterogeneous local data.

\iffalse
\revision{FedMLB augments a pathway to each of network blocks in a local model, where the structure and parameters of each branch are borrowed from the global model.
To show the effectiveness of this type of branching, we conduct the experiments for a variant type of hybrid branches.
To this end, we augment a branch from network blocks in a global model where the parameters of each branch are those of local model. 
We then train the local model based on the loss function in \eqref{eq:total_loss} using the main pathway and the hybrid pathways, denoted as $\text{FedMLB}_{\text{G} \rightarrow \text{L}}$.}

\revision{Table~\ref{tab:abl_branch_type} shows that employing hybrid pathway stemming from local model blocks on knowledge distillation outperforms the variant.
$\text{FedMLB}_{\text{G} \rightarrow \text{L}}$ are regularized so that the output of the global model and the output of the local model are the same as possible. 
While this has the advantage of preserving global knowledge, there is also a disadvantage that can interfere with learning new knowledge. 
On the other hand, $\text{FedMLB}_{\text{L} \rightarrow \text{G}}$ may mitigate this issue in that it regularizes the newly learned knowledge so that it makes sense globally.}
\fi


\subsection{Effect of hyperparameters in FedMLB}

\paragraph{Ablation study for loss function}
To show the effectiveness of the cross-entropy loss of the hybrid pathways $\mathcal{L}_H^{\text{CE}}$ and the KL-divergence loss $\mathcal{L}_H^{\text{KL}}$, we conduct the comprehensive experiments by varying $\lambda_1$ and $\lambda_2$ in \eqref{eq:total_loss}, which controls the weight of each of the two loss terms.
Table~\ref{tab:lambda_sensitivity} shows that both of the loss terms contribute to performance gains while the KL-divergence loss is more critical than the cross-entropy loss in the hybrid pathways.
%the use of only a single term clearly degrades accuracy.
%We can also observe that FedMLB shows results in terms of the choices of $\lambda_1$ and $\lambda_2$ on CIFAR-100 in moderate-scale federated learning setting.
Note that we set $\lambda_1 = \lambda_2 = 1$ in our experiment.

\paragraph{Softmax function temperature in knowledge distillation}
The temperature parameter $\tau^{\prime}$ in \eqref{eq:kl_loss} controls the smoothness of the softmax function output for KL divergence loss, $\mathcal{L}_H^{\text{KL}}$.
Table~\ref{tab:temperature_sensitivity} presents that the performance of FedMLB is consistent with respect to the variations of $\tau^\prime$ in the two different values of the symmetric Dirichlet parameter.
%This is partly because that overly smoothed output of softmax function may not transfer precise information of global information.



%


%%%%%%%%%%%%%%%%%%%%%%%%%% Acc / local computation
\begin{figure}[!t]
\vspace{11pt}
  \centering
\includegraphics[width=0.95\linewidth]{figures/acc_wrt_execution_time_w_title.pdf}
\caption{
%Performance evaluation of algorithms by varying their local computational costs.
Performance of algorithms by varying their local computational costs controlled by the number of local iterations while maintaining the total communication costs.
Accuracies are measured after $1K$ rounds on CIFAR-100 using ResNet18.}
\label{fig:local_iterations}
%\vspace{-2mm}
\end{figure}
%%%%%



\subsection{Local computation overheads}
%The calculation amount added by each auxilary pathway is less than the calculation amount of the main pathway. Therefore, please note that the total calculation is linear, not quadratic, with the number of pathways.
%FedMLB indeed requires extra local computation, but its benefit outweighs its cost as illustrated in Figure~\ref{fig:local_iterations}; 
While FedMLB requires additional computation compared to the baselines under the same number of local epochs, its benefit outweighs its cost as illustrated in Figure~\ref{fig:local_iterations}.
FedMLB outperforms other methods at the same computational cost and the gap gets more significant as they have more local iterations.
An important observation from Figure~\ref{fig:local_iterations} is that FedLS-NTD and FedGKD are inconsistent with the number of local iterations compared to FedMLB and FedAVG. Also, note that the performance of FedMLB improves substantially with more iterations, which is effective for reducing the communication cost, which is critical in federated learning.
Also, Table~\ref{tab:path_combinations} presents that removing a couple of pathways from deeper layers sometimes improves accuracy, which means there still exists room for optimization in terms of computational cost.


%%%%%%%%%%% Different DNN architectures
\begin{table}[t]
%\vspace{-8pt}
\centering
\caption{Results with different CNN backbone architectures on CIFAR-100.}
\vspace{1mm}
\label{tab:diff_arch}
\scalebox{0.9}{
%\setlength{\tabcolsep}{0.15cm} \hspace{-0.2cm}
\begin{tabular}{lcccc}
%\multirow{2}{*}{Method}          & \multicolumn{2}{c}{Dirichlet (0.3)}\\ 
%& {5$\%$, 100 clients } & {2$\%$, 100 clients }     \\ 
\multirow{2}{*}{Architecture}   &  \multicolumn{4}{c}{Dir(0.3), 100 clients, 5$\%$}\\ 
&FedAvg &FedLS-NTD & FedGKD  &FedMLB\\ %& FedAvg & FedMLB \\
\cline{1-5}
VGG-9               &47.04&51.37&48.62&\bf{54.54}\\%&30.99&36.87   \\
MobileNet           &38.52&47.66&47.72&\bf{48.34}\\%& \revision{10.27(408R)}& \revision{9.41(408R)}\\
ShuffleNet          &37.04	&39.27&38.47 &\bf{42.29}\\%	& \revision{19.11(374R)}	& \revision{21.8(374R)}\\
SqueezeNet          &39.86	&39.56&{42.28}&\bf{42.71}\\%	&\revision{23.38(742R)}	&\revision{21.9(742R)}\\
ResNet-18            &47.83&49.29 &47.96&\bf{54.58}\\%&37.48&42.61 \\
\cline{1-5}
\end{tabular}}
\vspace{-2mm}
\end{table}


\subsection{Experiments with other backbone models}
\iffalse
%Verification is conducted to confirm that FedMLB is effective in various architectures.
To confirm the generality of the benefits of FedMLB, we conduct experiments on various architectures.
VGG is widely used network without skip connections.
MobileNet, ShuffleNet, and SqueezeNet are lightweight networks suitable for edge devices.
For implementation, since these modern deep neural networks are typically modularized we branch a pathway after a module, \textit{e.g.}, ResBlock (no branches within a skip connection).
Table~\ref{tab:diff_arch} shows that FedMLB clearly outperforms other algorithms regardless of the backbone architectures which have fewer parameters  and computations.
%It is also effective for networks that have fewer parameters which is suitable for edge devices.
\fi
To confirm the generality of FedMLB with respect to backbone networks, we conduct experiments with additional architectures, which include VGG-9~\cite{simonyan2014very}, MobileNet~\cite{sandler2018mobilenetv2}, ShuffleNet~\cite{zhang2018shufflenet}, and SqueezeNet~\cite{iandola2016squeezenet}.
VGG is widely used network without skip connections while MobileNet, ShuffleNet and SqueezeNet are lightweight networks suitable for edge devices.
As for implementation, since these modern deep neural networks are typically modularized, we typically branch a pathway after a module, \textit{e.g.}, ResBlock (no branches from the layers enclosed by a skip connection).
Table~\ref{tab:diff_arch} shows that FedMLB clearly outperforms other algorithms regardless of the backbone architectures.





\iffalse
\subsection{Evaluation on less heterogeneous clients}
\revision{
\cref{tab:moderate_and_large_scales_dir06}~show the results of the experiment by changing the number of devices and the partition rate when the data distribution of the client is less heterogeneous. 
Compared to using only the existing method, the experimental results when using FedMLB together always show better performance with high margin. 
In addition, our method showed better performance when mass clients with low participation rates, which have difficulty in global convergence. 
For example, when FedMLB was added to Fedavg, the accuracy of relatively increasing is 17.5\% for moderated-scale setting, but 21.7\% for large-scale setting.}
\fi


%\input{tables/moderate_clients_dir06.tex}
%\input{tables/large_clients_dir06.tex}
%\input{tables/moderate_and_large_scales_dir06.tex}
%\input{tables/moderate_and_large_scales_IID.tex}


\iffalse
\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figures/Addwithbaseline_5.pdf}
\caption{5\% participation, 100 clients}
\end{subfigure}
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figures/Addwithbaseline_2.pdf}
\caption{2\% participation, 500 clients}
\end{subfigure}
\caption{The convergence plot of baselines and the result of combining FedMLB to them on CIFAR-100 with different ederated learning scenarios. The + symbol next to the baseline name refers to the result when combined with FedMLB.}
\label{fig:curve_baseline}
\end{figure*}


\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figures/KD_FitNet_5.pdf}
\caption{5\% participation, 100 clients}
\end{subfigure}
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figures/KD_FitNet_2.pdf}
\caption{2\% participation, 500 clients}
\end{subfigure}
\caption{The convergence plot of FedMLB and direct application of knowledge distillation on CIFAR-100 with different ederated learning scenarios.}
\label{fig:KD_FitNet}
\end{figure*}


\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figures/Feddistill_5.pdf}
\caption{5\% participation, 100 clients}
\end{subfigure}
\begin{subfigure}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{figures/Feddistill_2.pdf}
\caption{2\% participation, 500 clients}
\end{subfigure}
\caption{The convergence plot of FedMLB and regularization-based methods on CIFAR-100 with different ederated learning scenarios.}
\label{fig:curve_distil}
\end{figure*}

\fi


%\input{tables/moderate_clients_IID.tex}
%\input{tables/large_clients_IID.tex}



==> ICML arxiv/sections/introduction.tex <==
% !TEX root = ../main.tex

%%%%%%%%% INTRODUCTION
\section{Introduction}
\label{sec:introduction}

Training deep neural networks typically relies on centralized algorithms, where computing resources and training data are located within a single server.
Recently, to deal with large-scale models and/or distributed data, the learning frameworks based on multiple remote machines become widespread in machine learning research and development.
Federated learning~\cite{mcmahan2017communication} is a unique distributed learning framework that takes advantage of computing resources and training data in clients, typically edge devices, which is helpful to secure data privacy but often suffers from insufficient computing power, low communication bandwidth, and extra battery consumption.
As practical solutions to handle the challenges, each edge device often runs a small number of iterations and minimizes the communication rounds with the central server.

\iffalse
The number of edge devices is increasing explosively, and the amount of data accumulated therein is also increasing. 
Training a deep learning model using these data can bring a lot of usefulness to people, but sending distributed data to the server is not possible due to privacy issues.
Federated learning circumvents this problem by taking a different approach.
\fi


\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/framework_backprop_final.pdf}
\caption{Illustration of the local network for the proposed multi-level branched regularization framework. $B_L$ and $B_G$ denote network blocks extracted from local and global networks, respectively, and their superscripts indicate block indices. \iffalse $q_L$ \fi $q_L$ and $q_H$ indicate softmax outputs of the main pathway and hybrid pathways, respectively.
Solid and dashed gray lines represent forward and backpropagation flows, respectively.
For training, the standard cross-entropy losses are applied to all branches and the KL-divergence losses between the main pathway and the rest of the pathways are employed for regularization.
Note that we update the parameters in the main pathway only, which are illustrated in sky blue color in this figure.}
\label{fig:framework}
\end{figure}


FedAvg~\cite{mcmahan2017communication}, the standard optimization method of federated learning, maintains the global model in the server by aggregating the local models trained independently in multiple clients.
Each client utilizes its own dataset to update the local model instead of sharing the data with the server or other clients, sends the locally optimized model to the server for aggregation, and downloads the updated global model for the next stage.
%distributes the shared model from the server to the clients participating in the learning instead of sending data from each device. 
%Clients locally update the transmitted model using their own data multiple times and return the obtained local model back to the server. 
%A new shared model is obtained by aggregating local models obtained in this way.
%
FedAvg works well when the individual datasets of the clients are iid and the participation rate of the clients is high, but it struggles with low convergence speed otherwise. 
This is because, when the data distributions of individual clients are different from the global distribution, local updates are prone to drift and increase divergence with respect to the global model~\cite{zhao2018federated, karimireddy2019scaffold}.

\iffalse
In order to properly deal with client heterogeneity, this report proposes a method of using global data information in a shared global model for local training.
This method makes the features learned by the local model meaningful from the point of view of the global model.
Contraty to the existing methods that try to reduce only the loss between the label and the logit obtained by forwarding the image to the local model, proposed method reduce the loss between the label and the logit obtained by forwarding the intermediate local model features to the global model branch.
Also, it improves consistency by reducing the KL divergence between the logit obtained by multiple branches and the logit obtained by the local model.

The proposed method has the following advantages. 
First of all, the proposed method uses the information in the global model for local learning, but does not fall into the dilemma of failing to learn new knowledge because of preserving fixed knowledge.
Also, the proposed method does not require additional communication cost per round or additional memory spaces for storing local states compared to FedAvg.
Moreover, it can be used in parallel with other existing state of the art methods to improve performance.
\fi

\iffalse
\paragraph{\revision{[Motivation]}}
\revision{
Our goal is to preserve the global view from the latest global model against the model drift during independent local training in heterogeneous clients.
The shifting of the learned features occurs by over-fitting toward the biased local distribution during multiple local updates, and the updated local model no more represents the global distribution, which is sub-optimal for the global objective function in Eq~\ref{eq:global_objective}.}

\paragraph{\revision{[Overview]}}
\revision{In order to mitigate the information gaps among independent local models, we propose a novel knowledge distillation technique which utilize multi-level branches of the global model to prevent locally learned feature from being deviated from the feature space of the global model.}

\revision{A participating client first modularizes the downloaded global network into
multiple blocks based on the depth of layers and the feature map sizes.
\revision{The client trains the local model with the fixed global branches corresponding to individual blocks in the latest global model, where we minimize the differences in the representations between the global and the local branches by adding regularization terms in the local objective function.}
\fi

%
Our goal is to make each client preserve the latest global representations and prevent model drift caused by independent local updates.
Meanwhile, we make the server learn client-specific knowledge by a simple aggregation of local networks and achieve a high-performance model well-suited for all clients, eventually. 
To mitigate the discrepancy between the local models updated by heterogeneous datasets, we propose a novel architectural regularization technique via knowledge distillation that grafts the local and global subnetworks and constructs multi-level branches.
The auxiliary branches reduce the deviation of the representations in the local models from the feature space of the global model.
To this end, a participating client first modularizes the downloaded global network into
multiple blocks.
The client trains the main pathway of the local model with the parameters corresponding to the global subnetworks fixed, while the output representations of the hybrid pathways are made similar to those in the main pathway using additional regularization terms based on knowledge distillation.
Our regularization approach is unique compared to the methods based on the standard knowledge distillation because it constrains the representations of the main pathway in the local model using the on-the-fly outputs of the hybrid pathways.
This idea is motivated by a recent knowledge distillation approach that aims to learn a student-friendly teacher network~\cite{park2021learning}.
Figure~\ref{fig:framework} illustrates our main idea.

The main contributions of this work are as follows:
%
 \begin{itemize} 
%\item[$\bullet$]\revision{We propose a novel regularization technique, which prevents local model from drifting by constructing multiple branches and performing knowledge distillation between output of local model and global branches.}
\item[$\bullet$]We propose a simple but effective regularization technique to reduce the drift problem of a local model, via online knowledge distillation between the main pathway and the multiple hybrid pathways reflecting the global representations partially.
\item[$\bullet$]Our approach is robust to typical challenges of federated learning including data heterogeneity and low client participation rate, and is applicable to various federated learning frameworks.
\item[$\bullet$]The proposed method requires no additional communication cost and spends no extra memory to store the history of local or global states and the auxiliary information.
%, which is desirable for the real-world applications of federated learning.
\item[$\bullet$]We demonstrate through extensive experiments that our architectural regularization technique improves accuracy and convergence speed consistently compared to the state-of-the-art federated learning algorithms.
%that revise local objective function.}
 \end{itemize}
 %
 
The organization of this paper is as follows. 
We first discuss existing work related to the optimization in federated learning and review the basic concept with a simple solution in Section~\ref{sec:related} and \ref{sec:preliminaries}, respectively.
Section~\ref{sec:proposed} describes the proposed federated learning framework, and Section~\ref{sec:experiments} demonstrates the effectiveness of the proposed approach via extensive experiments.
Finally, we conclude this paper in Section~\ref{sec:conclusion}.

==> ICML arxiv/sections/method.tex <==
% !TEX root = ../main.tex

%%%%%%%%% PROPOSED METHOD


\section{Proposed Algorithm: FedMLB}
\label{sec:proposed}
%Our core target is to reduce local model drift through global model distillation. 
This section describes the details of our approach for federated learning with multi-level branched regularization, referred to as FedMLB, which exploits the representations of multiple hybrid pathways.


\subsection{Overview}
\label{sub:overview}
The main objective of FedMLB is to prevent the representations of the local model from being deviated too much by local updates while accommodating new knowledge from each client with heterogeneous datasets through independent local updates.
We achieve this goal via indirect layer-wise online knowledge distillation using the architecture illustrated in Figure~\ref{fig:framework}.

Although there exist several regularization approaches based on knowledge distillation for federated learning~\cite{lee2021preservation, yao2021local, zhu2021data}, FedMLB is unique in the sense that it constructs multiple hybrid pathways combining the subnetworks of local and global models at various levels and learns the representations of the local model similar to those of the hybrid pathways.
Note that the proposed approach performs knowledge distillation using on-the-fly targets given by the hybrid pathways although the subnetworks of the global model remain fixed.
%not based on the static global representations.
The regularization using the multiple auxiliary branches plays a critical role to make the individual blocks of the local network aligned well to the matching subnetworks of the global model.
%Assuming that the global model does not change significantly in a single round communication, the regularization is helpful to encourage consistent updates of local models despite their data homogeneity.
Consequently, local updates in each client allow the local model to be less deviated from the global counterpart, and such a regularization also reduces the variations of the models collected from multiple clients.
We describe the details of the proposed algorithm next.

\iffalse
\subsection{Motivation and overview}

\paragraph{\revision{[Motivation]}}
\revision{
Our goal is to preserve the global view from the latest global model against the model drift during independent local training in heterogeneous clients.
The shifting of the learned features occurs by over-fitting toward the biased local distribution during multiple local updates, and the updated local model no more represents the global distribution, which is sub-optimal for the global objective function in Eq~\ref{eq:global_objective}.}

\paragraph{\revision{[Overview]}}
\revision{In order to mitigate the information gaps among independent local models, we propose a novel knowledge distillation technique which utilize multi-level branches of the global model to prevent locally learned feature from being deviated from the feature space of the global model.}

\revision{A participating client first modularizes the downloaded global network into
multiple blocks based on the depth of layers and the feature map sizes. This is due to accurate extraction and transfer of global knowledge for the local training in local models.
Figure~\ref{fig:framework} presents the case that both networks are modularized into 3 blocks, denoted by ${B_L^1,B_L^2, B_L^3}$ and ${B_G^1,B_G^2, B_G^3}$ for a local model and global model, respectively.
}

\revision{The client trains the local model with the fixed global branches corresponding to individual blocks in the latest global model, where we minimize the differences in the representations between the global and the local branches by adding regularization terms in the local objective function.}
\fi



\subsection{Multi-level hybrid branching}
\label{sub:multi}

To perform the proposed regularization, we first divide the network into $M$ exclusive blocks, which are based on the depths and the feature map sizes of the architecture.
Let $\{B_L^m\}_{m=1}^M$ and $\{B_G^m\}_{m=1}^M$ be the sets of blocks in a local model and the global network, respectively.
The main pathway consists of local blocks $B_L^{1:M}$ and we create multiple hybrid pathways by augmenting a subnetwork in the global model $B_G^{m+1:M}$ to a local subnetwork $B_L^{1:m}$. 
%we create a hybrid pathway by augmenting a subnetwork in the global model $B_G^{m+1:M}$ to a local subnetwork $B_L^{1:m}$.
Depending on branching locations, from $1$ to $M-1$, several different hybrid pathways, denoted by $\{ B_L^{1:m}, B_G^{m+1:M} \}_{{m \in  \{1,\dots,M-1\}}}$, are constructed in parallel as illustrated in Figure~\ref{fig:framework}.

The constructed network by multi-level hybrid branching has $M$ pathways altogether for predictions, which includes one main pathway and $M-1$ hybrid pathways.
The softmax output of the main pathway, $q_L(x; \tau )$, is given by
%
\begin{equation}
 q_L(x; \theta, \tau) = \text{softmax} \left (\frac{f_L(x; \theta)}{\tau} \right), 
\end{equation}
%
where $x$ is the input of the network, $\theta$ is the model parameters, $\tau$ is the temperature of the softmax function, and $f_L(\cdot ; \cdot)$ denotes the logit of the main pathway.
Similarly, the softmax output of the hybrid pathway stemming from $B_L^m$ is given by
%
\begin{equation}
 q_H^m(x; \theta_m, \tau) =\text{softmax} \left (\frac{f_H^m(x ; \theta_m)}{\tau} \right), 
\end{equation}
%
where $f_H^m(\cdot ; \cdot)$ and $\theta_m$ denote the logit and the model parameter of the $m^\text{th}$ hybrid pathway, respectively.

\iffalse
\revision{
FedMLB is composed of a local model and multiple hybrid branches.
We divide the local model and the global model into $M$ blocks based on the depth of layers and feature map sizes, which are denoted by $\{B_L^m\}_{m=1}^M$ and $\{B_H^m\}_{m=1}^M$ for a local model and global model, respectively.
This is due to accurate extraction and transfer of global knowledge for the local model training.
Figure~\ref{fig:framework} presents the case that both networks are modularized into 3 blocks.
%Given an input $x$ of the network, we then construct $M-1$ global branches $R^j=\{B_G^m\}_{m=j+1}^M~(1\leq j \leq M-1)$ where intermediate local feature $F_L^j$ is forwarded to the corresponding global model branch $R^j$.
Given an input $x$ of the network, we then construct $M-1$ hybrid branches $R^j=\{B_H^m\}_{m=j+1}^M~(1\leq j \leq M-1)$ where deeper global blocks are is set after each shallow local block. 
In other words, intermediate local feature $F_L^j$ is forwarded to the corresponding hybrid branch $R^j$.
These hybrid branches are only utilized in training local models and can be removed in inference.}
\fi


\input{algorithms/proposed_method.tex}


\subsection{Knowledge distillation}
\label{sub:knowledge}

Our goal is to learn the representation of the main pathway similar to those of the hybrid pathways by using knowledge distillation.
To this end, we employ two different kinds of loss terms; one is the cross-entropy loss and the other is the knowledge distillation loss.

The cross-entropy loss of the main pathway is given by
%
\begin{equation}
    \mathcal{L}_L = \text{CrossEntropy}( q_L, y),
\label{eq:main_ce_loss}
\end{equation}
%
while the overall cross-entropy loss of the hybrid pathways is defined as
%
\begin{equation}
    \mathcal{L}_{H}^\text{CE} = \frac{1}{M-1} \sum_{m=1}^{M-1} \text{CrossEntropy}(q_H^m, y).
\label{eq:hybrid_ce_loss}
\end{equation}

On the other hand, we encourage the representations of individual hybrid pathways to be similar to the main branch of the local network and employ the following knowledge distillation loss additionally:
%
\begin{equation}
    \mathcal{L}_{H}^{\text{KL}} = \frac{1}{M-1} \sum_{m=1}^{M-1} {\text{KL}}(\tilde{q}_H^m, \tilde{q}_L),
\label{eq:kl_loss}
\end{equation}
%
where $\text{KL}(\cdot, \cdot)$ denotes the Kullback-Leibler (KL) divergence between two normalized vectors, and $\tilde{q}$ is the temperature-scaled softmax output using the hyperparameter $\tilde{\tau}$.\iffalse$\tilde{\tau} (> \tau)$ \revision{ (\geq \tau)$}.\fi

The total loss function of the proposed method is given by
%
\begin{equation}
\mathcal{L} = \mathcal{L}_{L} + \lambda_1 \cdot \mathcal{L}_H^{\text{CE}} + \lambda_2 \cdot \mathcal{L}_H^{\text{KL}},
\label{eq:total_loss}
\end{equation}
%
where $\lambda_1$ and $\lambda_2$ are hyperparameters that determine the weights of individual terms.



\iffalse
\revision{
% To prevent the model drift during local training in skewed data distribution,  to preserve the global view from the latest global model against the model drift during independent local training in heterogeneous clients.
We utilize the logits from the multi-level branches to bridge the gap between the representations learned by the local model and the global model. 
Our local loss function is composed of three terms: local task loss in the local model $\mathcal{L}_L$, cross-entropy loss $\mathcal{L}_{H}^\text{CE}$ in the hybrid branch, and Kullback-Leibler loss $L_{H}^{\text{KL}}$ in the hybrid branch.}

\revision{Each loss term is defined as follows. First, $\mathcal{L}_L$ is given by the cross-entropy between the local model's
prediction $q_L$ and the ground-truth label $y$ as
\begin{equation}
    \mathcal{L}_L = \text{CrossEntropy}(q_L, y).
\end{equation}
We also minimize error between the hybrid branch logits and the ground-truth, which is obtained by the average cross-entropy loss from all the hybrid branches as}
\begin{equation}
    \mathcal{L}_{H}^\text{CE} = \frac{1}{M-1} \sum_{m=1}^{M-1} \text{CrossEntropy}(q_H^m, y),
\end{equation}
\revision{where $q_H^j$ denotes logits obtained from $j$-th hybrid branch. Note that we set temperature to 1 for the both cross entropy loss $\mathcal{L}_L$ and $\mathcal{L}_{H}^\text{CE}$.
This term enforces the learned representation with skewed data not to lose representations of global model.
Therefore, this regularization term has the effect of learning global-aware features that preserve representation of global distribution.}

\revision{In addition, we also employ the Kullback–Leibler divergence between $q_H^j$ and $q_L$, where $M-1$ hybrid branches are considered together as}
\begin{equation}
\label{KL}
    \mathcal{L}_{H}^{\text{KL}} = \frac{1}{M-1} \sum_{j=1}^{M-1} {\text{KL}}(\tilde{q}_H^j,\tilde{q}_L),
\end{equation}
\revision{
where $\tilde{q}_H^j$ and $\tilde{q}_L$ are outputs of a softmax function having a larger temperature $\tau^\prime$.
The total loss function of the proposed method is given by}
%
\begin{equation}
\label{proposed_loss}
\mathcal{L} = \mathcal{L}_{L} + \lambda_1 \cdot \mathcal{L}_H^{\text{CE}} + \lambda_2 \cdot \mathcal{L}_H^{\text{KL}},
\end{equation}
%
\revision{where $\lambda_1$ and $\lambda_2$ are hyperparameters that determine the weights of individual terms. 
Note that we do not update global blocks in global branches.}
\fi

The local model is optimized by backpropagation based on the loss function in \eqref{eq:total_loss}.
Note that we update the model parameters in the main pathway while the blocks from the global network in the hybrid pathways remain unchanged during the local updates.



\subsection{Learning procedure}
\label{sub:learning}

Our federated learning follows the standard protocol and starts from local updates in clients.
Each client first builds a model with either pretrained or randomized parameters and updates the parameters for a small number of iterations using local data.
The updated models are sent to the server, and the server aggregates the models by a simple model averaging.
Since the communication between the server and the clients is not stable, only a small fraction of clients typically participate in each round of the training procedure.
Finally, the server broadcasts the new model given by model averaging and initiates a new round.
Note that FedMLB is a client-side optimization approach and there is no special operation in the server.
Algorithm~\ref{alg:proposed_method} describes the detailed learning procedure of FedMLB.


\input{tables/moderate_and_large_scales}




\subsection{Discussion}
\label{sub:discussion}

FedMLB maintains the knowledge in the global model while accommodating new information from the client datasets in each communication round.
This objective is similar to that of continual learning, and knowledge distillation (KD) is widely used to this end.
However, vanilla KD-based methods~\cite{lee2021preservation,yao2021local} match the representations at the logit level, which derives model updates primarily at deeper layers while the parameters in the lower layers are less affected.
This issue can be alleviated by using the layer-wise KD techniques~\cite{romero2014fitnets}, but the independent supervisions at multiple layers may lead to inconsistent and restrictive updates of model parameters.
Contrary to these two options, the proposed approach constructs separate pathways using the static network blocks of the global model and updates the representations in each block of the local model to induce the proper outputs of the network.
At the same time, FedMLB effectively distributes the workload of the network across multiple blocks for adapting to the local data, which is helpful for maintaining the representations of the global model during local iterations.


\iffalse
FedMLB can be categorized as a knowledge distillation approach for federated learning, but it is different from the standard knowledge distillation mainly because it attempts to fit the local model to moving targets given by the hybrid pathways.
The standard knowledge distillation would not be a good solution for federated learning due to the following two reasons.
First, the global model, which plays a role as a teacher, is not fully optimized and the optimization towards the global model leads to a suboptimal solution.
Second, even though we can trust the representations of the global model, the additional loss for knowledge distillation restricts the flexibility of local models excessively. 
In particular, since each client has heterogeneous datasets, a single teacher model (the global model) may not be able to provide sufficient room for accommodating diverse client-specific updates, leading to slow convergence of the global model.
\fi

\iffalse
Another possible interpretation of the proposed design is model augmentation; each client learns invariant representations to minor variations in the model parameters.
Such a network is trained by the regularization through multi-level auxiliary branches.
The model augmentation has a similar motivation to the network design for self-supervised contrastive learning without using negative examples~\cite{grill2020bootstrap,chen2021exploring}, where the network with two branches have slightly different architectures to learn robust representations without collapsing to degenerate models.
\fi

Compared to the federated learning techniques that handle client heterogeneity by employing global gradient information for the local update, the proposed algorithm has the following major advantages.
First, FedMLB does not require any additional communication overhead such as global gradient information~\cite{karimireddy2019scaffold, xu2021fedcm}. 
Note that the increase in communication cost challenges many realistic federated learning applications involving clients with limited network bandwidths.
Also, unlike~\cite{karimireddy2019scaffold, acar2020federated, li2021model}, the clients are not supposed to store their local states or historical information of the model, which is particularly desirable for the low-rate participation situations in federated learning.

Meanwhile, FedMLB incurs a moderate increase of computational cost due to the backpropagation through the additional branches.
However, it achieves impressive accuracy with fewer communication rounds compared to the baselines.
The performance of FedMLB is particularly good with a relatively large number of local iterations, which is helpful for reducing the number of communication rounds even further to achieve the target accuracy.
%However, our experimental results in Table~\ref{tab:lambda_sensitivity} show that FedMLB without the cross-entropy loss in the hybrid pathways still show competitive performance while reducing the backpropagation cost greatly.

\iffalse
\subsection{Overview}

In the existing method, the local model is trained only with the goal of reducing the loss on local data. 
Because the client's data is limited, the local model learned on the local data is overfitted, and the features of the local model and the features of the global model can be completely different semantically. 
In this case, the features created by the local model will not contain useful information from the point of view of the global model.
On the other hand, the proposed methods train the local model to find features that contain useful information even in the view of the global model.


\subsection{Modularizing global and local models}
First of all, each client keeps a frozen copy of the global model shared in this communication round while doing local iterations.
Then, the global model and local model are divided into $M$ blocks. At this time, since the architectures of the two models are the same, the dividing point is the same.
\cref{fig:long} presents the case that both networks are modularized into 3 blocks, denoted by ${B_L^1,B_L^2, B_L^3}$ and ${B_G^1,B_G^2, B_G^3}$ for a local model and global model , respectively.

\subsection{Global model branches}
In the proposed method, the local model generates features and local model logit by forwarding the image.
In \cref{fig:long}, features are ${F_L^1,F_L^2, F_L^3}$ and local model logit is $q_L$. 
All intermediate features are forwarded to the global model branch, except for the last feature used directly to create local logit.
This is like finding the logit when forwarding the image using a model in which the parameters of the front block of the model are of the local model and the parameters of the rear block are of the global model.
This global branch logits $q_G^i$ show the results of the global model interpretation of local features.
Since global branches are composed of parameters of the shared global model, additional communication costs are not required.
And since global branches are used only for model training and not for inference, there is no need for additional computational cost during inference.
\fi

==> ICML arxiv/sections/preliminary.tex <==
% !TEX root = ../main.tex

%%%%%%%%% PRELIMINARY

\section{Preliminaries}
\label{sec:preliminaries}
This section briefly discusses the concept and procedure of the basic federated learning algorithm.

\subsection{Problem setting and notations}
%\paragraph{\revision{[Federated learning task]}}
%Suppose that there exist $N$ clients for a task of federated learning.
%The goal of the federated learning task is to learn a global model $\theta$ that minimizes the average losses of all clients as follows:
Given $N$ clients, the goal of the federated learning is to learn a global model $\theta$ that minimizes the average losses of all clients as follows:
%
\begin{equation}
\label{eq:global_objective}
    \underset{\theta }{\text{argmin}} \left[ \mathcal{L}(\theta) = \frac{1}{N} \sum_{i=1}^N \mathcal{L}_i(\theta) \right],
\end{equation}
%
where $\mathcal{L}_i(\theta)=\mathbb{E}_{{(x,y)} \sim D_i}[ \mathcal{L}_i(x,y;  \theta)]$ is the loss in the $i^\text{th}$ client given by the expected loss over all instances in the client, denoted by $D_i$.
Note that clients may have heterogeneous data distributions and exchanges of training data are strictly prohibited due to privacy issues. 
%In this paper, we will use the notations in~\cref{tab:notation} to describe our algorithm.
%
%\input{tables/notation.tex}


\subsection{FedAvg algorithm}
%\paragraph{\revision{[Fedavg and its difficulties encountered with non iid and partly participation ]}}
FedAvg~\cite{mcmahan2017communication} is a standard solution of federated learning, where the server simply aggregates all the participating client models to obtain the global model.
Specifically, in the $t^\text{th}$ communication round, a central server first sends a global model $\theta^{t-1}$ to each of the clients.
Each client sets its initial parameter $\theta^{t}_{i, 0}$ to $\theta^{t-1}$, \textit{i.e.}, $\theta_{i, 0} = \theta^{t-1}$,  performs $K$ steps of the gradient descent optimization to minimize its local loss, and then returns the resultant model parametrized by $\theta_{i,K}^t$ to the server. 
An updated global model for the next round training is obtained by averaging all the participating local models in the current communication round. 
The local loss of FedAvg at the $k^\text{th}$ local iteration ($k = 1, \dots, K$) is defined by
%
\begin{equation}
\label{fedavg_loss}
    \mathcal{L}_i(\theta_{i,k}^t) = \mathbb{E}_{{(x,y)} \sim D_i}[\mathcal{L}_i(x,y ; \theta_{i,k}^t)],
\end{equation}
%
where the cross-entropy loss is typically used for $\mathcal{L}_i$.
\iffalse
The local model update is given by
%
\begin{equation}
\theta_{i,k}^t \leftarrow \theta_{i,k-1}^t - \eta \nabla \mathcal{L}_i,
\label{eq:local_update_fedavg}
\end{equation}
%
where $\eta$ is a hyperparameter.
%\input{algorithms/fedavg.tex}
%
\fi

Multiple local updates in FedAvg before the aggregation step in the server decreases the communication cost for training apparently.
However, in practice, it typically leads to the so-called client drift issue~\cite{karimireddy2019scaffold}, where the individual client updates are prone to be inconsistent due to overfitting on local client data. 
This phenomenon inhibits FedAvg from converging to the optimum of the average loss over all clients.

==> ICML arxiv/sections/related_work.tex <==
% !TEX root = ../main.tex

%%%%%%%%% RELATED WORK
\section{Related Work}
\label{sec:related}
Federated learning~\cite{mcmahan2017communication} is a distributed learning framework with the characteristics such as non-iid client data, data privacy requirement, massive distribution, and partial participation.
Although FedAvg provides a practical solution for the issues, it still suffers from the heterogeneity of data across clients~\cite{zhao2018federated}.
On the theoretical side, there exist several works that derive convergence rates with respect to the data heterogeneity~\cite{li2020federated, wang2019adaptive, khaled2019first, li2019convergence, hsieh2020non, wang2020tackling}.

%In this work, we focus on the problem of the features learned during local training are overfitted only to local data.

%\paragraph{\revision{[Regularization based approaches.]}}
\iffalse 
To alleviate the limitations of FedAvg, several works aim to prevent local models from drifting towards local minima by regularizing their local objectives.
These approaches regularize the client loss function by adding a proximal term~\cite{li2020federated} in local loss function, employing control variates~\cite{karimireddy2019scaffold, li2019feddane}, or using primal-dual approaches~\cite{zhang2020fedpd, acar2020federated}.
In activation regularization perspective, client update is regularized to have similar activation to the downloaded global model by contrastive learning~\cite{li2021model}, using mixup with global statistics~\cite{yoon2021fedmix}, and using generative models~\cite{zhu2021data}. 
 All of these existing methods are regularized so that the output of the global model and the output of the local model are the same as possible. While this has the advantage of preserving global knowledge, there is also a disadvantage that can interfere with learning new knowledge. On the other hand, the proposed method is different in that it regularizes the newly learned knowledge so that it makes sense globally.
\fi

To alleviate the limitations of FedAvg, the local model updates are often regularized to prevent a large deviation from the global model. 
FedProx~\cite{li2020federated} imposes a quadratic penalty over the distance between the server and client parameters
%Others use a form of variance reduction techniques such as control variates~\cite{karimireddy2019scaffold, li2019feddane}, or penalize each client's risk objective dynamically based on its local gradient~\cite{zhang2020fedpd, acar2020federated}.
while SCAFFOLD~\cite{karimireddy2019scaffold} and FedDANE~\cite{li2019feddane} employ a form of variance reduction techniques such as control variates.
On the other hand, FedPD~\cite{zhang2020fedpd} and FedDyn~\cite{acar2020federated} penalize each client's risk objective dynamically based on its local gradient.
\iffalse To alleviate the limitations of FedAvg, the local model updates are often regularized for reducing the deviation of local networks from the global model using proximal terms~\cite{li2020federated}, control variates~\cite{karimireddy2019scaffold, li2019feddane}, or primal-dual analysis~\cite{zhang2020fedpd, acar2020federated}. \fi
Some approaches adopt a trick motivated by data augmentation~\cite{yoon2021fedmix}\ghkim{,} or contrastive learning~\cite{li2021model} to ensure the similarity of the representations between the downloaded global model and local networks.
%\bh{Other works enforce local models to have similar activation to the downloaded global model by adopting mixup with global statistics~\cite{yoon2021fedmix} or model-level contrastive learning~\cite{li2021model}.}
However, these methods typically rely on unrealistic or impractical assumptions such as high participation rates, additional communication costs, or extra memory requirements in clients.


Meanwhile, the server-side optimization techniques have been discussed actively for the acceleration of the convergence.
For example, FedAvgM~\cite{hsu2019measuring} adds a momentum term to speed up training, and FedADAM~\cite{reddi2021adaptive} adopts an adaptive gradient-descent method.
Our approach and these aggregation-based methods are orthogonal, so combining them together can yield additional performance gains.

There is another line of research that utilizes knowledge distillation to tackle data heterogeneity issue  in federated learning.
The algorithms in this category perform knowledge distillation either in the server or clients.
As client distillation methods, FD~\cite{seo2020federated} shares the representations between clients for knowledge distillation with their ensemble features while FedLS-NTD~\cite{lee2021preservation} transfers the knowledge of the global model to local networks except the activations for ground-truth labels.
FedGKD~\cite{yao2021local} employs representations from the ensemble of the historical global models to refine local models, and FedGen~\cite{zhu2021data} learns a global generator to aggregate the local information and distill global knowledge to clients.
For the distillation in the server, FedDF~\cite{lin2020ensemble} utilizes the averaged representations of local models on proxy data for aggregation.
However, these methods require additional communication overhead~\cite{yao2021local, zhu2021data} or auxiliary data~\cite{seo2020federated, lin2020ensemble}.
In particular, as discussed in~\cite{wang2021field}, federated learning algorithms are sensitive to the communication cost and the use of globally-shared auxiliary data should be cautiously performed. 
To the contrary, our approach incurs no additional communication cost and has no requirement of auxiliary data.
The proposed algorithm belongs to the method for local optimization based on knowledge distillation.

\iffalse
\revision{[Knowledge distillation methods] There is another line of work which utilize knowledge distillation techniques in federated learning to handle data heterogeneity problem.
%Knowledge distillation is proposed to transfer knowledge from an expert teacher model to a student model.
Most approaches based on knowledge distillation aim to make the global model learn the ensemble of locally trained models. 
For instance, a few works collect logits from local models to regularize local training~\cite{seo2020federated} or for distillation at server aggregation~\cite{chen2020fedbe, lin2020ensemble}.
Logits from the latest global model are also utilized to regularize local model~\cite{lee2021preservation, yao2021local}.
Besides, FedGen~\cite{zhu2021data} learns a global generator to aggregate the local information and distills global knowledge to users.
However, these works require additional communication overhead~\cite{yao2021local, zhu2021data} or auxiliary data~\cite{seo2020federated, chen2020fedbe, lin2020ensemble}.
As discussed in~\cite{wang2021field}, federated learning algorithms are particularly sensitive to the communication cost, and using globally-shared auxiliary data should be cautiously generated or collected. 
In contrary, our approach does not require any additional information to communicate or auxiliary data.
}
\fi
\iffalse
There is another line of work focusing on reducing inter-client variance to eliminate inconsistent update across clients.
several approaches use control variates~\cite{karimireddy2019scaffold, liang2019variance, karimireddy2020mime, li2019feddane} or global gradient momentum~\cite{xu2021fedcm} to reduce bias in client update.
\cite{khanduri2021stem, das2020faster} apply STORM algorithm~\cite{cutkosky2019momentum} to reduce variance caused by both server-level and client-level SGD procedures.
Another way to de-bias client updates is to estimate the global posterior using local posterior sampling by running Markov chain Monte Carlo (MCMC) in client side~\cite{al2020federated}.
However, most of these methods require full participation, additional communication cost or client storage, which can be problematic in realistic federated learning tasks.
\fi



==> ICML arxiv/tables/Feddistill.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$, 100 clients}                                                                     & \multicolumn{4}{c}{2$\%$, 500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\% & 500R           & \multicolumn{1}{c}{1000R}    & 30\%         & 36\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.54  & 47.57  & 428 & 939  & 29.87& 37.48& 504& 858 \\
FedProx~\cite{li2020federated}                      & 42.03  & 47.93  & 419 & 886 & 29.28 & 36.16 & 533 & 966  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 386 &  740 & 28.66 &35.99  & 546 & 1000+  \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 397 & 872  & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
FedMLB                                                & \bf{47.39} & \bf{54.58} & \bf{339} & \bf{488} & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> ICML arxiv/tables/KD_FitNet.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparisons between FedMLB and the baselines with the standard knowledge distillation techniques on CIFAR-100. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_kd}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$, 100 clients}                                                                     & \multicolumn{4}{c}{2$\%$, 500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\% & 500R           & \multicolumn{1}{c}{1000R}    & 30\%         & 36\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.54  & 47.57  & 428 & 939  & 29.87& 37.48& 504& 858 \\
FedAvg + KD~\cite{hinton2014distilling}             & {42.99}  & {49.17}  & {389} & {752}   & {29.83} & {37.65}  & {505} & {859}  \\
FedAvg + FitNet~\cite{romero2014fitnets}          &  42.04 & 47.67  & 419 &914   & 29.92 &37.63  &503  & 860  \\
FedMLB                                                & \bf{47.39} & \bf{54.58} & \bf{339} & \bf{488} & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> ICML arxiv/tables/LFGN.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Ablation study results from two different compositions of the hybrid pathways on CIFAR-100 in two federated learning settings.
% \bhb{where the symmetric Dirichlet parameter for non-iid sampling is 0.3.}
The accuracy at the target round and the number of communication rounds to reach the target test accuracy are based on the exponential moving average with the momentum parameter $0.9$. 
%The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.
}
\label{tab:abl_branch_type}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{Dir(0.3), 100 clients, 5$\%$}                                                                     & \multicolumn{4}{c}{Dir(0.3), 500 clients, 2$\%$}                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 48\% & 500R           & \multicolumn{1}{c}{1000R}    & 30\%         & 36\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 428 & 1000+  & 29.87& 37.48& 504& 858 \\
%FedAvg + KD~\cite{hinton2014distilling}             & {42.99}  & {49.17}  & {389} & {752}   & {29.83} & {37.65}  & {505} & {859}  \\
%FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 434 &1000+   & 28.89 &36.11  &995  & 995  \\
%\cdashline{1-9}
%FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 425 & 881 & 29.28 & 36.16 & 533 & 966  \\
%FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 386 &  740 & 28.66 &35.99  & 546 & 1000+  \\
%MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{550} & \revision{875}  &  &  &  &   \\
%FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 397 & 872  & 29.27 & 37.25 & 530&896  \\
$\text{FedMLB}_{\text{G} \rightarrow \text{L}}$     & 42.41  & 47.40  & 386 & 1000+  & 28.53 & 35.46 & 571& 1000+  \\
$\text{FedMLB}_{\text{L} \rightarrow \text{G}}$ (ours)     & \bf{47.39} & \bf{54.58} & \bf{339} & \bf{523} & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-9}
\end{tabular}}
\vspace{-0.3cm}
\end{table*}

==> ICML arxiv/tables/avgacc_numofbranches.tex <==
\begin{table}[t]
    \centering
    %\vspace{-6.5pt}
    \captionof{table}{
    %\jkkim{Average accuracy after $1K$ rounds of FedMLB according to used numbers of branches on CIFAR-100 in the moderate-scale setting}.
    %\bhr{Average accuracy after $1K$ rounds  of FedMLB by varying the number of branches used on CIFAR-100 in the moderate-scale setting}.
    Effect of the number of hybrid pathways employed for FedMLB on CIFAR-100 in the moderate-scale setting. 
The average accuracy and the standard deviation are computed over all possible combinations with the same number of hybrid pathways.
We measure the accuracy after 1$K$ rounds, where the symmetric Dirichlet parameter is set to 0.3 for  non-iid sampling.
%\ghkim{Average accuracy after $1K$ rounds for all possible combinations of pathways of FedMLB by varying the number of pathways used on CIFAR-100 in the moderate-scale setting.}
%     \jkkim{The Dirichlet parameter is set to 0.3.}
    }
    \vspace{0.1cm}
    \label{tab:avgacc_numofbranches}
    \scalebox{0.9}{
    \setlength{\tabcolsep}{2mm}
    \hspace{-0.3cm}
    \begin{tabular}{cccccc}
		%\hline
%		\multicolumn{5}{c}{Hybrid pathway index} & \multicolumn{1}{c||}{100 clients} & \multirow{2}{*}{\# of pathways} & \multirow{2}{*}{Avg acc.} \\
%                1 &2 &3 &4 &5 & Dir(0.3), 5$\%$ &  \\

                %\cline{1-6}
                Number of pathways &1&2&3&4&5\\\cline{1-6}
                Average accuracy &47.89&51.86& 52.89& 53.69 & \bf{54.58} \\              
                Standard deviation &\ \ 3.99&\ \ 2.45& \ \ 1.78& \ \ 1.43 & - \\              
                %Num. of pathways &5&4&3&2&1\\\cline{1-6}
               %Avg acc. &54.58&53.69& 52.89& 51.86 & 47.89

                \cline{1-6}
                             
	\end{tabular}
	}
\vspace{-0.2cm}
\end{table}

==> ICML arxiv/tables/dummy.tex <==
% !TEX root = ../main.tex
%
\iffalse
\begin{table*}[h]
\centering
\caption{Comparison of federated learning methods on CIFAR-100: Dirichlet (0.6) split on 5\% client participation out of 100 clients. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:abl_dir06}
\scalebox{0.9}{
\begin{tabular}{lcccc} 
%\cline{1-13}
%& \multicolumn{8}{c}{Local epochs}  \\
%\cline{2-9}

\cline{2-5}
 \multirow{2}{*}{Methods} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 54\% & 58\%                \\ 
\cline{1-5}
FedAvg~\cite{mcmahan2017communication} & 43.91 & 49.18& 1000+ &1000+  \\
FedProx~\cite{li2020federated}                 & 43.15 &48.45 &1000+ &  1000+ \\
FedAvgm~\cite{hsu2019measuring}               &46.66  & 52.49 & 1000+ & 1000+  \\
FedAdam~\cite{reddi2021adaptive}              &45.95 & 51.63 & 1000+& 1000+ \\
FedDyn~\cite{acar2020federated}                  & 53.74 &59.70 & 518&   776   \\
FedCM~\cite{xu2021fedcm}                            &53.75 &60.48 & 511&    740   \\
FedAGM                                              &{58.82} &{63.88} & {325}&  {471} \\
Ours                                              &  {49.25} & {56.26}  & {757} & {1000+} \\
Ours + FedAGM                                              &  \bf{62.29} & \bf{66.79}  & \bf{276} & \bf{349} \\
\cline{1-5}
\end{tabular}}
\end{table*}

\begin{table*}[t]
\centering
\caption{Comparison of federated learning methods when the number of local iterations is 100 on CIFAR-100: Dirichlet (0.3) split on 5\% client participation out of 100 clients. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:abl_local_iterations}
\scalebox{0.9}{
\begin{tabular}{lcccc} 
%\cline{1-13}
%& \multicolumn{8}{c}{Local epochs}  \\
%\cline{2-9}
 Local iterations & \multicolumn{4}{c}{$K$ = 100}  \\ 
\cline{2-5}
 \multirow{2}{*}{Methods} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\%                \\ 
\cline{1-5}
FedAvg~\cite{mcmahan2017communication} &41.92 & 48.16  & 896 & 1000+  \\
FedProx~\cite{li2020federated}                 &  42.01 & 48.17  & 888 &  1000+ \\
FedAvgm~\cite{hsu2019measuring}               &  45.72 &  52.74 & 578 & 1000+  \\
FedAdam~\cite{reddi2021adaptive}              &  43.00 &  47.51 & 994  &  1000+ \\
FedDyn~\cite{acar2020federated}                  &  51.98 & 59.13  &347  & 532   \\
FedCM~\cite{xu2021fedcm}                            &  46.90 & 54.20  & 502 & 893  \\
FedAGM                                              &  {54.71} & {63.12}  & {284} & {461} \\
Ours                                              &  {52.53} & {58.52}  & {341} & {525} \\
Ours + FedAGM                                              &  \bf{57.62} & \bf{65.89}  & \bf{238} & \bf{357} \\
\cline{1-5}
\end{tabular}}
\end{table*}
\fi


==> ICML arxiv/tables/hybrid_pathways.tex <==
%%%%%%%%%%% Subset of branches
\iffalse
\begin{table}[t]
    \centering
    \vspace{-6.5pt}
    \captionof{table}{
    Accuracy after $1K$ rounds of FedMLB with various configurations of the hybrid pathways.
    }
    \vspace{0.1cm}
    \label{tab:path_combinations}
    \scalebox{0.9}{
    \setlength{\tabcolsep}{2.2mm}
    %\hspace{-0.2cm}
    \begin{tabular}{cccccc||cc}
		%\hline
%		\multicolumn{5}{c}{Hybrid pathway index} & \multicolumn{1}{c||}{100 clients} & \multirow{2}{*}{\# of pathways} & \multirow{2}{*}{Avg acc.} \\
%                1 &2 &3 &4 &5 & Dir(0.3), 5$\%$ &  \\
		\multicolumn{5}{c}{Hybrid pathway index} & \multirow{2}{*}{Acc.} & Num. of & \multirow{2}{*}{Avg acc.} \\
                1 &2 &3 &4 &5 &  & pathways & \\
                \cline{1-8}
                 \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & 54.58 & 5 & 54.58 \\ \cline{1-6}
                 \checkmark  & \checkmark  & \checkmark  & \checkmark  &             & 55.18 & 4 & 53.69  \\
                 \checkmark  & \checkmark  & \checkmark  &             &             & 55.03 & 3 & 52.89 \\
                 \checkmark  & \checkmark  &             &             &             & 54.16 & 2 & 51.86  \\
                 \checkmark  &             &             &             &             & 50.79 & 1 & 47.89 \\ \cline{1-6}
                 %\cline{1-6}
                             &             &             &             & \checkmark  & 48.45& 0 & 47.83  \\
                             &             &             & \checkmark  & \checkmark  & 46.78&  &  \\
                             &             & \checkmark  & \checkmark  & \checkmark  & 51.73 & \multicolumn{2}{c}{100 clients, Dir(0.3), 5$\%$} \\
                             & \checkmark  & \checkmark  & \checkmark  & \checkmark  & 52.65 & \multicolumn{2}{c}{CIFAR-100, ResNet-18} \\
	\end{tabular}
	}
%\vspace{-0.3cm}
\end{table}
\fi

\begin{table}[t]
    \centering
    %\vspace{-6.5pt}
    \captionof{table}{
    Accuracy after $1K$ rounds of FedMLB with various configurations of the hybrid pathways on CIFAR-100 in the moderate-scale setting.
    The symmetric Dirichlet parameter is set to 0.3.
    }
    \vspace{0.1cm}
    \label{tab:path_combinations}
    \scalebox{0.9}{
    \setlength{\tabcolsep}{5mm}
    %\hspace{-0.2cm}
    \begin{tabular}{cccccc}
		%\hline
%		\multicolumn{5}{c}{Hybrid pathway index} & \multicolumn{1}{c||}{100 clients} & \multirow{2}{*}{\# of pathways} & \multirow{2}{*}{Avg acc.} \\
%                1 &2 &3 &4 &5 & Dir(0.3), 5$\%$ &  \\
		\multicolumn{5}{c}{Hybrid pathway index} & \multirow{2}{*}{Acc.}  \\
                1 &2 &3 &4 &5 &  \\
                \cline{1-6}
                 \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & 54.58 \\ \cdashline{1-6}
                 \checkmark  & \checkmark  & \checkmark  & \checkmark  &             & 55.18   \\
                 \checkmark  & \checkmark  & \checkmark  &             &             & 55.03  \\
                 \checkmark  & \checkmark  &             &             &             & 54.16   \\
                 \checkmark  &             &             &             &             & 50.79  \\ \cdashline{1-6}
                 %\cline{1-6}
                             &             &             &             & \checkmark  & 48.45  \\
                             &             &             & \checkmark  & \checkmark  & 46.78  \\
                             &             & \checkmark  & \checkmark  & \checkmark  & 51.73  \\
                             & \checkmark  & \checkmark  & \checkmark  & \checkmark  & 52.65  \\ \cline{1-6}
	\end{tabular}
	}
\vspace{-0.2cm}
\end{table}





==> ICML arxiv/tables/lambdaCE_analysis.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{$\mathcal{L}_{G}^\text{CE}$ analysis}
\label{tab:local_approaches}
\scalebox{0.9}{
\begin{tabular}{ccccc} 
%\cline{1-13}
\multirow{3}{*}{$\mathcal{L}_{G}^\text{CE}$}                                   & \multicolumn{3}{c}{5$\%$,100 clients}   \\                                                                                                                                                                                                                
\cline{2-5}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}   \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\%  \\ 
\cline{1-5}
0.75                & 29.87& 37.48& 504& 858 \\
1                & {29.83} & {37.65}  & {505} & {859}  \\
1.25            & 28.89 &36.11  &551  & 995  \\
1.5                      & 29.28 & 36.16 & 533 & 966  \\
2                 & 28.66 &35.99  & 546 & 1000+  \\
3                              & \revision{38.36}  & \revision{48.61}  & \revision{550} & \revision{875}    \\
5                            & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
10                                                 & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-5}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> ICML arxiv/tables/lambdaKL_analysis.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{$\mathcal{L}_{G}^{\text{KL}}$ analysis}
\label{tab:local_approaches}
\scalebox{0.9}{
\begin{tabular}{ccccc} 
%\cline{1-13}
\multirow{3}{*}{$\mathcal{L}_{G}^{\text{KL}}$}                                   & \multicolumn{3}{c}{5$\%$,100 clients}   \\                                                                                                                                                                                                                
\cline{2-5}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}   \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\%  \\ 
\cline{1-5}
0.75                & 29.87& 37.48& 504& 858 \\
1                & {29.83} & {37.65}  & {505} & {859}  \\
1.25            & 28.89 &36.11  &551  & 995  \\
1.5                      & 29.28 & 36.16 & 533 & 966  \\
2                 & 28.66 &35.99  & 546 & 1000+  \\
3                              & \revision{38.36}  & \revision{48.61}  & \revision{550} & \revision{875}    \\
5                            & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
10                                                 & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-5}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> ICML arxiv/tables/lambda_analysis.tex <==
% !TEX root = ../main.tex

\begin{table}[t]
\centering
\caption{Sensitivity of FedMLB to the weights of the two regularization loss terms with respect to the accuracy after 1$K$ round on CIFAR-100 in the moderate-scale setting. The symmetric Dirichlet parameter is set to 0.3.}


\label{tab:lambda_sensitivity}
\vspace{0.1cm}
\scalebox{0.9}{
%\resizebox{\columnwidth}{!}{

\begin{tabular}{c|cccc} 
%\cline{1-13}
\backslashbox{$\lambda_1$}{$\lambda_2$}          & 0 & 1& 2& 3  \\     
\cline{0-4}
0               & 47.83 &  53.27 & 54.51 & 54.21 \\
%0.5            & 51.63 & 54.05 & 54.61 & 54.55 & 54.80 \\
1               & 52.10 &  54.58 &55.52 & \bf{56.32}   \\     
2               & 52.37 &  53.05 & 54.28 & 54.16  \\  
3               & 49.54 & 53.00 & 54.34 & 53.57  \\  
\cline{0-4}
\end{tabular}}
\vspace{-0.2cm}
\end{table}

==> ICML arxiv/tables/large_clients.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a large number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 500, 2\%, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:large_clients}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 36\% & 40\% & 500R           & \multicolumn{1}{c}{1000R}    & 26\%         & 32\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 29.87& 37.48& 858& 1000+ &23.63  & 29.48  & 645 &  1000+ \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvg + FedMLB                           & \bf{32.03} & \bf{42.61}  & \bf{642} & \bf{800} &{\bf28.39} & {\bf33.67}  & {\bf429} & {\bf710} \\
\cline{1-9}
FedAvgm~\cite{hsu2019measuring}                & 31.80 & 40.54 & 724 & 955 & 26.75 & 33.26  & 457 & 836  \\
FedAvgm + FedMLB                           & \bf{36.21} & \bf{47.75}  & \bf{496} & \bf{636} &{\bf32.00} & {\bf37.53}  & {\bf307} & {\bf500} \\
\cline{1-9}
FedAdam~\cite{reddi2021adaptive}                & 36.07 & 47.04 & 480 & 653  & 29.65 & 35.91  & 345  & 642  \\
FedAdam + FedMLB                          & \bf{38.28} & \bf{52.68}  & \bf{442} & \bf{527} &{\bf32.14} & {\bf39.54}  & {\bf311} & {\bf524} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}                   & 31.58 & 41.02 & 691 & 927  &24.35 & 29.54  & 595 & 1000+   \\
FedDyn + FedMLB                           & \bf{36.50} & \bf{49.65}  & \bf{478} & \bf{611} &{\bf30.77} & {\bf37.68}  & {\bf384} & {\bf541} \\
\cline{1-9}
\end{tabular}}
\end{table*}

==> ICML arxiv/tables/large_clients_IID.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a large number of clients with IID distribution. In these experiments, the number of clients and participation rate are set to 500 and 2\%, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:large_clients_IID}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 36\% & 44\% & 500R           & \multicolumn{1}{c}{1000R}    & 26\%         & 32\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  &{29.96}& {36.93}& {903}  & {1000+} & 23.25  & 28.92 & 701 & 1000+   \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvg + FedMLB                           & \bf{34.60} &\bf{ 44.95}  & \bf{549} & \bf{ 935} & \bf{28.27} &\bf{ 35.51} &\bf{ 435} &\bf{ 689} \\
\cline{1-9}
FedAvgM~\cite{hsu2019measuring}         & 32.47 & 41.04  & 679 &  1000+ & 27.52 & 34.08 & 445 & 800 \\
FedAvgM + FedMLB                          &\bf{ 38.60} &\bf{50.52}   & \bf{418} & \bf{676}  & \bf{33.51} &  & \bf{281} &\bf{444}  \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}        &38.32  &  48.70 & 430 & 712  &  &  & 252 & 441 \\
FedADAM + FedMLB                          &\bf{42.48} &  \bf{55.24} &\bf{338}  &\bf{539 }  &  &  & \bf{250} & \bf{384 }\\
\cline{1-9}
FedDyn~\cite{acar2020federated}         &  35.77& 47.34  & 509 &  806 & 24.79 &  &565  &  \\
FedDyn + FedMLB                           & \bf{39.37} & \bf{53.11}  & \bf{429} & \bf{619}  & \bf{30.46} & \bf{37.89 }& \bf{384} & \bf{540} \\
\cline{1-9}
\end{tabular}}
\end{table*}

==> ICML arxiv/tables/large_clients_dir06.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a large number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 500, 2\%, and $0.6$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:large_clients_dir06}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 29.36 &  36.36 &  966& 1000+  & 24.48 & 29.94 & 600 & 1000+ \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvg + FedMLB                           &\bf{33.74}  & \bf{43.53}  & \bf{571} & 1000+  & \bf{28.97} & \bf{35.08} & \bf{415} & \bf{650} \\
\cline{1-9}
FedAvgM~\cite{hsu2019measuring}         & 32.44 & 41.40  & 680 & 1000+  & 24.65 & 31.54 & 575 & 1000+ \\
FedAvgM + FedMLB                          & \bf{38.35} & \bf{49.65} & \bf{421} & \bf{690}  & \bf{32.33} & \bf{37.6} & \bf{308} & \bf{483} \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}        & 37.33 &  47.73 & 463 &756   & 31.4 & 37.03 & \bf{286} & 876 \\
FedADAM + FedMLB                           &\bf{39.57}  & \bf{53.53}  & \bf{402} & \bf{621}  & \bf{33.71} & \bf{41.15} & 292 & \bf{619} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}         & 31.63 & 41.58  & 677 & 1000+  & 26.42 & 31.80 & 485 & 1000+ \\
FedDyn + FedMLB                          & \bf{38.90} & \bf{52.72}  & \bf{440} & \bf{639}  & \bf{32.52} & \bf{38.28} & \bf{350} & \bf{712} \\\cline{1-9}
\end{tabular}}
\end{table*}

==> ICML arxiv/tables/local_approaches.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison between FedMLB and the baselines based on other local objectives on CIFAR-100 with two different federated learning settings.
% \bhb{when the non-iid data are simulated using a symmetric Dirichlet distribution parametrized by 0.3.}
The accuracy at the target round and the number of communication rounds to reach the target test accuracy are based on the exponential moving average with the momentum parameter $0.9$. 
%The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.
}
\label{tab:local_approaches}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{Dir(0.3), 100 clients, 5$\%$}                                                                     & \multicolumn{4}{c}{Dir(0.3), 500 clients , 2$\%$}                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 48\% & 500R           & \multicolumn{1}{c}{1000R}    & 30\%         & 36\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 428 & 1000+  & 29.87& 37.48& 504& 858 \\
FedAvg + KD~\cite{hinton2014distilling}             & {42.99}  & {49.17}  & {389} & {842}   & {29.83} & {37.65}  & {505} & {859}  \\
%FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 434 &1000+   & 28.89 &36.11  &551  & 995  \\
%FedAvg + FitNets~\cite{}          &   &  &  &   &  &  &  &   \\
FedAvg + FitNet~\cite{romero2014fitnets}          &  42.04 & 47.67  & 419 & 1000+   & 29.92 &37.63  &503  & 860  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.03  & 47.93  & 419 & 1000+ & 29.28 & 36.16 & 533 & 966  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 386 &  825 & 28.66 &35.99  & 546 & 1000+  \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 397 & 1000+  & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
FedMLB (ours)                                                & \bf{47.39} & \bf{54.58} & \bf{339} & \bf{523} & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-9}
\end{tabular}}
\vspace{-0.2cm}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of FedMLB with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> ICML arxiv/tables/local_approaches_IID.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\% & 500R           & \multicolumn{1}{c}{1000R}    & 30\%         & 36\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 924  & 29.87& 37.48& 504& 858 \\
FedAvg + KD~\cite{hinton2014distilling}             & {42.99}  & {49.17}  & {389} & {752}   & {29.83} & {37.65}  & {505} & {859}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 434 &1000+   & 28.89 &36.11  &551  & 995  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 425 & 881 & 29.28 & 36.16 & 533 & 966  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 386 &  740 & 28.66 &35.99  & 546 & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{550} & \revision{875}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 397 & 872  & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{339} & \bf{488} & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> ICML arxiv/tables/local_approaches_dir06.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\% & 500R           & \multicolumn{1}{c}{1000R}    & 30\%         & 36\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 924  & 29.87& 37.48& 504& 858 \\
FedAvg + KD~\cite{hinton2014distilling}             & {42.99}  & {49.17}  & {389} & {752}   & {29.83} & {37.65}  & {505} & {859}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 434 &1000+   & 28.89 &36.11  &551  & 995  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 425 & 881 & 29.28 & 36.16 & 533 & 966  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 386 &  740 & 28.66 &35.99  & 546 & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{550} & \revision{875}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 397 & 872  & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{339} & \bf{488} & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> ICML arxiv/tables/low_participation.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-10 and CIFAR-100 with low participation rates (1\%). In these experiments, the number of clients and Dirichlet parameter are set to 100, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10} & \multicolumn{4}{c}{CIFAR-100} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 46.72 & 64.33 &  &   &  &  &  &  \\
FedAvg + Ours                           & 37.45 & 57.24 &  &  & &  &  &  \\
\cline{1-9}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}         & 46.05 & 63.73  &  &   &  &  &  &   \\
FedAvgm + Ours                          & 41.41 & 43.25  &  &   &  &  &  & \\
\cline{1-9}
FedAdam~\cite{reddi2021adaptive}        & 37.42 & 51.94  &  &  &  &  &  &   \\
FedAdam + Ours                          & 19.76 & 23.78 &  &  &  &  &  &  \\
\cline{1-9}
FedDyn~\cite{acar2020federated}         & 50.60 & 68.72 &  &   &  &  &  &   \\
FedDyn + Ours                           & 41.41 & 64.54  &  &   &  &  &  &  \\
\cline{1-9}
\end{tabular}}
\end{table*}



==> ICML arxiv/tables/moderate_and_large_scales.tex <==
% !TEX root = ../main.tex
%


\begin{table*}[t]
\centering
\caption{Comparisons between FedMLB and the baselines on CIFAR-100 and Tiny-ImageNet for two different federated learning settings.  For (a) moderate-scale experiments, the number of clients and the participation rate are set to 100 and 5\%, respectively, while (b) large-scale experiments have 500 clients with 2\% participation rate. The accuracy at the target round and the number of communication rounds to reach the target test accuracy are based on the exponential moving average with the momentum parameter $0.9$. The arrows indicate whether the higher ($\uparrow$) or the lower ($\downarrow$) is better. }
%The best performance in each column is marked in {\bf bold}.
\label{tab:moderate_and_large_scales}
%\vspace{0.1cm}
\begin{subtable}[t]{1\textwidth}
\centering
\captionof{table}{Moderate-scale with Dir(0.3): 100 clients, 5\% participation}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 38\%         & 42\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 33.94 & 35.42  &  1000+& 1000+ \\
%FedAvg + FedMLB                                              & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} &{\bf37.20} & {\bf40.16}  & {\bf539}& {1000+} \\
FedMLB                                              & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} &{\bf37.20} & {\bf40.16}  & {\bf539}& {1000+} \\
\cline{1-9}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgM~\cite{hsu2019measuring}                & 46.98  & 53.24  & 515 & 936  & 36.10 & 38.36  & 794& 1000+  \\
FedAvgM + FedMLB                                             & \bf{53.02} & \bf{58.97} & \bf{349} & \bf{499} & {\bf40.93} & {\bf43.52} & {\bf380}& {\bf642}  \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}                & 47.07  & {54.19}  & 499 & 947  & \bf{36.98} & 40.60 & 647 &  1000+ \\
FedADAM + FedMLB                                              & \bf{48.59} & \bf{58.23} & \bf{472} &\bf{645} & {35.81} & {\bf42.90}  & {\bf552}& {\bf873} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}                  & 48.38  & 55.78  & 425 & 735
&37.35&41.17&573&1000+ \\
FedDyn + FedMLB                                              & \bf{57.33} & \bf{61.81} & \bf{299} & \bf{377} &{\bf43.05} & {\bf46.55}  & {\bf324}& {\bf446} \\
\cline{1-9}\end{tabular}}
\end{subtable}


\vspace{0.3cm}
\begin{subtable}[t]{1\textwidth}
\centering
\captionof{table}{Large-scale with Dir(0.3): 500 clients, 2\% participation} 
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 36\% & 40\% & 500R           & \multicolumn{1}{c}{1000R}    & 26\%         & 32\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 29.87& 37.48& 858& 1000+ &23.63  & 29.48  & 645 &  1000+ \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
%FedAvg + FedMLB                           & \bf{32.03} & \bf{42.61}  & \bf{642} & \bf{800} &{\bf28.39} & {\bf33.67}  & {\bf429} & {\bf710} \\
FedMLB                           & \bf{32.03} & \bf{42.61}  & \bf{642} & \bf{800} &{\bf28.39} & {\bf33.67}  & {\bf429} & {\bf710} \\
\cline{1-9}
FedAvgM~\cite{hsu2019measuring}                & 31.80 & 40.54 & 724 & 955 & 26.75 & 33.26  & 457 & 836  \\
FedAvgM + FedMLB                           & \bf{36.21} & \bf{47.75}  & \bf{496} & \bf{636} &{\bf32.00} & {\bf37.53}  & {\bf307} & {\bf500} \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}                & 36.07 & 47.04 & 480 & 653  & 29.65 & 35.91  & 345  & 642  \\
FedADAM + FedMLB                          & \bf{38.28} & \bf{52.68}  & \bf{442} & \bf{527} &{\bf32.14} & {\bf39.54}  & {\bf311} & {\bf524} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}                   & 31.58 & 41.02 & 691 & 927  &24.35 & 29.54  & 595 & 1000+   \\
FedDyn + FedMLB                           & \bf{36.50} & \bf{49.65}  & \bf{478} & \bf{611} &{\bf30.77} & {\bf37.68}  & {\bf384} & {\bf541} \\
\cline{1-9}
\end{tabular}}
\end{subtable}
\end{table*}








==> ICML arxiv/tables/moderate_and_large_scales_IID.tex <==
% !TEX root = ../main.tex
%


\begin{table*}[h!!]
\centering
\caption{Comparisons of FedMLB and the baselines on CIFAR-100 and Tiny-ImageNet for two different iid federated learning settings. 
%For a moderate-scale experiment (a), the number of clients and participation rate, are set to 100, and 5\%, respectively, while a large-scale experiment (b) has 500 clients with 2\% participation rate. 
The accuracy at the target round and the number of communication rounds to reach the target test accuracy are based on the exponential moving average with the momentum parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better.
}
\label{tab:moderate_and_large_scales_IID}
%\vspace{0.1cm}
\begin{subtable}[t]{1\textwidth}
\centering
\captionof{table}{Moderate-scale with IID: 100 clients, 5\% participation}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 48\% & 52\% & 500R           & \multicolumn{1}{c}{1000R}    & 38\%         & 42\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 43.60 &  48.01 &  997& 1000+  & 37.96 & 38.92 & 504 & 1000+ \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvg + FedMLB                           &\bf{50.12}  &\bf{56.40  }&\bf{426} &\bf{584  }& \bf{40.69} & \bf{42.98} & \bf{376} & \bf{640} \\
\cline{1-9}
FedAvgM~\cite{hsu2019measuring}         & 47.43 & 52.83  & 532 & 880  & 39.79 & 41.34 & 346 & 1000+ \\
FedAvgM + FedMLB                          & \bf{55.29} & \bf{61.16}  & \bf{294} & \bf{377  }& \bf{44.02} & \bf{47.03} & \bf{271 }& \bf{382} \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}        & 54.35 &  60.35 & 303 &416   & 43.54 &  46.12& \bf{257} & 377 \\
FedADAM + FedMLB                           &\bf{57.13}  & \bf{62.58}  & \bf{285} & \bf{363 } & \bf{44.27} &\bf{47.36} &276  &\bf{372} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}         & 50.37 & 56.88  & 397 & 592  & 39.49 &  42.42& 350 & 848 \\
FedDyn + FedMLB                           & \bf{56.97 }& \bf{61.41}  & \bf{298} & \bf{366}  & \bf{44.28} & \bf{46.62} & \bf{277} & \bf{361} \\
\cline{1-9}
\end{tabular}}
\end{subtable}


\vspace{0.3cm}
\begin{subtable}[t]{1\textwidth}
\centering
\captionof{table}{Large-scale with IID: 500 clients, 2\% participation} 
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 36\% & 44\% & 500R           & \multicolumn{1}{c}{1000R}    & 26\%         & 32\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  &{29.96}& {36.93}& {903}  & {1000+} & 23.25  & 28.92 & 701 & 1000+   \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvg + FedMLB                           & \bf{34.60} &\bf{44.95}  & \bf{549} & \bf{ 935} & \bf{28.27} &\bf{35.51} &\bf{435} &\bf{ 689} \\
\cline{1-9}
FedAvgM~\cite{hsu2019measuring}         & 32.47 & 41.04  & 679 &  1000+ & 27.52 & 34.08 & 445 & 800 \\
FedAvgM + FedMLB                          &\bf{38.60} &\bf{50.52}   & \bf{418} & \bf{676}  & \bf{33.51} & \bf{39.37} & \bf{281} &\bf{444}  \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}        &38.32  &  48.70 & 430 & 712  & 33.30 & 37.55 & 252 & 441 \\
FedADAM + FedMLB                          &\bf{42.48} &  \bf{55.24} &\bf{338}  &\bf{539}  & \bf 35.34 & \bf 41.75 & \bf{250} & \bf{384 }\\
\cline{1-9}
FedDyn~\cite{acar2020federated}         &  35.77& 47.34  & 509 &  806 & 24.79 & 31.75 &565  &1000+  \\
FedDyn + FedMLB                           & \bf{39.37} & \bf{53.11}  & \bf{429} & \bf{619}  & \bf{30.46} & \bf{37.89 }& \bf{384} & \bf{540} \\
\cline{1-9}
\end{tabular}}
\end{subtable}
\end{table*}








==> ICML arxiv/tables/moderate_and_large_scales_dir06.tex <==
% !TEX root = ../main.tex
%


\begin{table*}[h!]
\centering
\caption{Comparisons of FedMLB and the baselines on CIFAR-100 and Tiny-ImageNet for two different  federated learning settings, where the symmetric Dirichlet parameter is 0.6.
%For (a) a moderate-scale experiment, the number of clients and participation rate, are set to 100, and 5\%, respectively, while a large-scale experiment (b) has 500 clients with 2\% participation rate. 
The accuracy at the target round and the number of communication rounds to reach the target test accuracy are based on the exponential moving average with the momentum parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better.
}
\label{tab:moderate_and_large_scales_dir06}
%\vspace{0.1cm}
\begin{subtable}[t]{1\textwidth}
\centering
\captionof{table}{Moderate-scale with Dir(0.6): 100 clients, 5\% participation}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 48\% & 52\% & 500R           & \multicolumn{1}{c}{1000R}    & 38\%         & 42\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 43.43 & 48.71  & 926 & 1000+  & 36.15 & 37.72 & 1000+ & 1000+ \\
FedMLB                           & \bf{49.36} & \bf{56.70}  & \bf{465} & \bf{602}  & \bf{39.34} & \bf{42.15} & \bf{441} & \bf{917} \\
\cline{1-9}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgM~\cite{hsu2019measuring}                & 46.66 & 52.49  & 572 &  937 & 38.41 & 40.75 & 475 & 1000+ \\
FedAvgM + FedMLB                                  & \bf{54.62} & \bf{60.91} & \bf{331} & \bf{417}  & \bf{43.96} & \bf{46.82} & \bf{294} & \bf{401} \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}                &50.81  &  56.95 & 427 & 569  & 40.13 & 42.75 & 415 & 813 \\
FedADAM + FedMLB                                  & \bf{53.34} & \bf{61.49}  & \bf{364} & \bf{467}  & \bf{40.67} & \bf{44.96} & 415 & \bf{610} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}                  &50.51  &56.79   & 427 & 580  & 39.39 & 42.97 & 423 & 875 \\
FedDyn + FedMLB                                  & \bf{57.51}  & \bf{62.43}   & \bf{298}  & \bf{355}  & \bf{43.35} & \bf{47.43} & \bf{294} & \bf{412} \\
\cline{1-9}
\end{tabular}}
\end{subtable}


\vspace{0.3cm}
\begin{subtable}[t]{1\textwidth}
\centering
\captionof{table}{Large-scale with Dir(0.6): 500 clients, 2\% participation} 
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 36\% & 44\% & 500R           & \multicolumn{1}{c}{1000R}    & 26\%         & 32\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 29.36 &  36.36 &  966& 1000+  & 24.48 & 29.94 & 600 & 1000+ \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedMLB                           &\bf{33.74}  & \bf{43.53}  & \bf{571} & 1000+  & \bf{28.97} & \bf{35.08} & \bf{415} & \bf{650} \\
\cline{1-9}
FedAvgM~\cite{hsu2019measuring}         & 32.44 & 41.40  & 680 & 1000+  & 24.65 & 31.54 & 575 & 1000+ \\
FedAvgM + FedMLB                          & \bf{38.35} & \bf{49.65} & \bf{421} & \bf{690}  & \bf{32.33} & \bf{37.60} & \bf{308} & \bf{483} \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}        & 37.33 &  47.73 & 463 &756   & 31.40 & 37.03 & \bf{286} & 533 \\
FedADAM + FedMLB                           &\bf{39.57}  & \bf{53.53}  & \bf{402} & \bf{621}  & \bf{33.71} & \bf{41.15} & 292 & \bf{444} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}         & 31.63 & 41.58  & 677 & 1000+  & 26.42 & 31.80 & 485 & 1000+ \\
FedDyn + FedMLB                          & \bf{38.90} & \bf{52.72}  & \bf{440} & \bf{639}  & \bf{32.52} & \bf{38.28} & \bf{350} & \bf{712} \\\cline{1-9}
\end{tabular}}
\end{subtable}
\vspace{-0.15cm}
\end{table*}








==> ICML arxiv/tables/moderate_clients.tex <==
% !TEX root = ../main.tex
%
\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR10, CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients}
\scalebox{0.9}{
\begin{tabular}{lcccccccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-13}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-13}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 33.94 & 35.42 & 645 &  1000+ \\
FedAvg + Ours                                              & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} &{\bf37.20} & {\bf40.16} & {\bf414} & {\bf539} \\
\cline{1-13}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgM~\cite{hsu2019measuring}                & 46.98  & 53.24  & 515 & 936  & 36.10 & 38.36  & 794& 1000+  \\
FedAvgm + Ours                                             & \bf{53.02} & \bf{58.97} & \bf{349} & \bf{499} & {\bf40.93} & {\bf43.52} & {\bf309} & {\bf380} \\
\cline{1-13}
FedAdam~\cite{reddi2021adaptive}                & 44.80  & \bf{52.48}  & 691 & 1000+  & 33.22 & 38.91 &  658& 945  \\
FedAdam + Ours                                              & \bf{46.04} & {51.12} & \bf{653} & {1000+} & {\bf33.49} & {\bf38.93} & {\bf640} & {\bf785} \\
\cline{1-13}
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 317 & 521  & 38.86 & 42.82 & 327 & 440  \\
FedDyn + Ours                                              & \bf{57.33} & \bf{61.81} & \bf{299} & \bf{377} &{\bf43.05} & {\bf46.55} & {\bf283} & {\bf324} \\
\cline{1-13}
\end{tabular}}
\end{table*}
\fi


\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is marked in {\bf bold}.}
\label{tab:moderate_clients}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 38\%         & 42\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 33.94 & 35.42  &  1000+& 1000+ \\
FedAvg + FedMLB                                              & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} &{\bf37.20} & {\bf40.16}  & {\bf539}& {1000+} \\
\cline{1-9}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgM~\cite{hsu2019measuring}                & 46.98  & 53.24  & 515 & 936  & 36.10 & 38.36  & 794& 1000+  \\
FedAvgm + FedMLB                                             & \bf{53.02} & \bf{58.97} & \bf{349} & \bf{499} & {\bf40.93} & {\bf43.52} & {\bf380}& {\bf642}  \\
\cline{1-9}
FedAdam~\cite{reddi2021adaptive}                & 47.07  & {54.19}  & 499 & 947  & \bf{36.98} & 40.6 & 647 &  1000+ \\
FedAdam + FedMLB                                              & \bf{48.59} & \bf{58.23} & \bf{472} &\bf{645} & {35.81} & {\bf42.9}  & {\bf552}& {\bf873} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}                  & 48.38  & 55.78  & 425 & 735
&37.35&41.17&573&1000+ \\
FedDyn + FedMLB                                              & \bf{57.33} & \bf{61.81} & \bf{299} & \bf{377} &{\bf43.05} & {\bf46.55}  & {\bf324}& {\bf446} \\
\cline{1-9}\end{tabular}}
\end{table*}






\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of federated learning methods on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_CIFAR_100}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 30.16& 38.11& 842& 1000+ \\
FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}                & 46.98  & 53.29  & 515 & 936  & 31.80 & 40.54 & 724 & 955  \\
FedAdam~\cite{reddi2021adaptive}                & 44.80  & 52.48  & 691 & 1000+  & 24.40 & 30.83 & 1000+ & 1000+  \\
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 293 & 504  & 33.52 & 45.01 & 576 & 714  \\
FedCM~\cite{xu2021fedcm}                            & 52.44  & 58.06  & 293 & 572  & 27.23 & 38.79 & 872 & 1000+ \\
FedAGM                                              & {57.04}  & {62.79}  & {245} & {353} & {35.68} & {48.40}  & {505} & {616}  \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {47.39} & {54.58} & {488} & {783} &{32.03} & {42.61}  & {642} & {800} \\
Ours + FedAGM                                              & \bf{61.32} & \bf{65.67} & \bf{216} & \bf{279} &\bf{41.10} & \bf{55.27}  & \bf{402} & \bf{479} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\begin{table*}[h]
\centering
\caption{Comparison of federated learning methods on Tiny-ImageNet with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_Tiny_ImageNet}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 35\% & 38\% & 500R           & \multicolumn{1}{c}{1000R}    & 24\%         & 30\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 33.94 & 35.42 & 645 &  1000+&23.63  & 29.48  & 523 &  1000+ \\
FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvgm~\cite{hsu2019measuring}                & 36.32 & 38.51 & 416 & 829 & 26.75 & 33.26  & 386 & 687  \\
FedAdam~\cite{reddi2021adaptive}                & 33.22 & 38.91 &  658& 945  & 21.88 & 28.08  & 648  & 1000+  \\
FedDyn~\cite{acar2020federated}                   & 38.86 & 42.82 & 327 & 440  & 27.74 & 37.25  & 387 & 580   \\
FedCM~\cite{xu2021fedcm}                            & 31.61 & 37.87 & 694 & 1000+ & 19.41 & 24.09  & 975 &  1000+ \\
FedAGM                                              & {42.26} & {46.31} & {226} & {331} &{31.47} & {38.48}  & {246} & {447} \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {37.20} & {40.16} & {414} & {539} &{28.39} & {33.67}  & {384} & {489} \\
Ours + FedAGM                                              & \bf{46.11} & \bf{50.54} & \bf{205} & \bf{260} &\bf{35.92} & \bf{43.85}  & \bf{209} & \bf{313} \\
\cline{1-9}
\end{tabular}}
\end{table*} 
\fi

==> ICML arxiv/tables/moderate_clients_IID.tex <==
% !TEX root = ../main.tex
%
\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR10, CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients}
\scalebox{0.9}{
\begin{tabular}{lcccccccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-13}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-13}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 33.94 & 35.42 & 645 &  1000+ \\
FedAvg + Ours                                              & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} &{\bf37.20} & {\bf40.16} & {\bf414} & {\bf539} \\
\cline{1-13}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}                & 46.98  & 53.29  & 515 & 936  & 36.32 & 38.51 & 416 & 829  \\
FedAvgm + Ours                                             & \bf{53.02} & \bf{58.97} & \bf{349} & \bf{499} & {\bf40.93} & {\bf43.52} & {\bf309} & {\bf380} \\
\cline{1-13}
FedAdam~\cite{reddi2021adaptive}                & 44.80  & \bf{52.48}  & 691 & 1000+  & 33.22 & 38.91 &  658& 945  \\
FedAdam + Ours                                              & \bf{46.04} & {51.12} & \bf{653} & {1000+} & {\bf33.49} & {\bf38.93} & {\bf640} & {\bf785} \\
\cline{1-13}
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 317 & 521  & 38.86 & 42.82 & 327 & 440  \\
FedDyn + Ours                                              & \bf{57.33} & \bf{61.81} & \bf{299} & \bf{377} &{\bf43.05} & {\bf46.55} & {\bf283} & {\bf324} \\
\cline{1-13}
\end{tabular}}
\end{table*}
\fi


\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients and participation rate are set to 100 and 5\% with IID distribution. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients_IID}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 48\% & 52\% & 500R           & \multicolumn{1}{c}{1000R}    & 38\%         & 42\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 43.60 &  48.01 &  997& 1000+  & 37.96 & 38.92 & 504 & 1000+ \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvg + FedMLB                           &\bf{50.12}  &\bf{ 56.40  }&\bf{ 426} &\bf{ 584  }& \bf{40.69} & \bf{42.98} & \bf{376} & \bf{640} \\
\cline{1-9}
FedAvgM~\cite{hsu2019measuring}         & 47.43 & 52.83  & 532 & 880  & 39.79 & 41.34 & 346 & 1000+ \\
FedAvgM + FedMLB                          & \bf{55.29} & \bf{61.16}  & \bf{294} & \bf{377  }& \bf{44.02} & \bf{47.03} & \bf{271 }& \bf{382} \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}        & 54.35 &  60.35 & 303 &416   & 43.54 &  46.12& \bf{257} & 377 \\
FedADAM + FedMLB                           &\bf{57.13}  & \bf{62.58}  & \bf{285} & \bf{363 } & \bf{44.27} &\bf{ 47.36} &276  &\bf{ 372} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}         & 50.37 & 56.88  & 397 & 592  & 39.49 &  42.42& 350 & 848 \\
FedDyn + FedMLB                           & \bf{56.97 }& \bf{61.41}  & \bf{298} & \bf{366}  & \bf{44.28} &  & \bf{277} & \bf{361} \\
\cline{1-9}\end{tabular}}
\end{table*}





\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of federated learning methods on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_CIFAR_100}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 30.16& 38.11& 842& 1000+ \\
FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}                & 46.98  & 53.29  & 515 & 936  & 31.80 & 40.54 & 724 & 955  \\
FedAdam~\cite{reddi2021adaptive}                & 44.80  & 52.48  & 691 & 1000+  & 24.40 & 30.83 & 1000+ & 1000+  \\
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 293 & 504  & 33.52 & 45.01 & 576 & 714  \\
FedCM~\cite{xu2021fedcm}                            & 52.44  & 58.06  & 293 & 572  & 27.23 & 38.79 & 872 & 1000+ \\
FedAGM                                              & {57.04}  & {62.79}  & {245} & {353} & {35.68} & {48.40}  & {505} & {616}  \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {47.39} & {54.58} & {488} & {783} &{32.03} & {42.61}  & {642} & {800} \\
Ours + FedAGM                                              & \bf{61.32} & \bf{65.67} & \bf{216} & \bf{279} &\bf{41.10} & \bf{55.27}  & \bf{402} & \bf{479} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\begin{table*}[h]
\centering
\caption{Comparison of federated learning methods on Tiny-ImageNet with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_Tiny_ImageNet}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 35\% & 38\% & 500R           & \multicolumn{1}{c}{1000R}    & 24\%         & 30\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 33.94 & 35.42 & 645 &  1000+&23.63  & 29.48  & 523 &  1000+ \\
FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvgm~\cite{hsu2019measuring}                & 36.32 & 38.51 & 416 & 829 & 26.75 & 33.26  & 386 & 687  \\
FedAdam~\cite{reddi2021adaptive}                & 33.22 & 38.91 &  658& 945  & 21.88 & 28.08  & 648  & 1000+  \\
FedDyn~\cite{acar2020federated}                   & 38.86 & 42.82 & 327 & 440  & 27.74 & 37.25  & 387 & 580   \\
FedCM~\cite{xu2021fedcm}                            & 31.61 & 37.87 & 694 & 1000+ & 19.41 & 24.09  & 975 &  1000+ \\
FedAGM                                              & {42.26} & {46.31} & {226} & {331} &{31.47} & {38.48}  & {246} & {447} \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {37.20} & {40.16} & {414} & {539} &{28.39} & {33.67}  & {384} & {489} \\
Ours + FedAGM                                              & \bf{46.11} & \bf{50.54} & \bf{205} & \bf{260} &\bf{35.92} & \bf{43.85}  & \bf{209} & \bf{313} \\
\cline{1-9}
\end{tabular}}
\end{table*} 
\fi

==> ICML arxiv/tables/moderate_clients_dir06.tex <==
% !TEX root = ../main.tex
%
\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR10, CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients}
\scalebox{0.9}{
\begin{tabular}{lcccccccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-13}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-13}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 33.94 & 35.42 & 645 &  1000+ \\
FedAvg + Ours                                              & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} &{\bf37.20} & {\bf40.16} & {\bf414} & {\bf539} \\
\cline{1-13}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}                & 46.98  & 53.29  & 515 & 936  & 36.32 & 38.51 & 416 & 829  \\
FedAvgm + Ours                                             & \bf{53.02} & \bf{58.97} & \bf{349} & \bf{499} & {\bf40.93} & {\bf43.52} & {\bf309} & {\bf380} \\
\cline{1-13}
FedAdam~\cite{reddi2021adaptive}                & 44.80  & \bf{52.48}  & 691 & 1000+  & 33.22 & 38.91 &  658& 945  \\
FedAdam + Ours                                              & \bf{46.04} & {51.12} & \bf{653} & {1000+} & {\bf33.49} & {\bf38.93} & {\bf640} & {\bf785} \\
\cline{1-13}
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 317 & 521  & 38.86 & 42.82 & 327 & 440  \\
FedDyn + Ours                                              & \bf{57.33} & \bf{61.81} & \bf{299} & \bf{377} &{\bf43.05} & {\bf46.55} & {\bf283} & {\bf324} \\
\cline{1-13}
\end{tabular}}
\end{table*}
\fi


\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and $0.6$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients_dir06}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 48\% & 52\% & 500R           & \multicolumn{1}{c}{1000R}    & 38\%         & 42\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 43.43 & 48.71  & 926 & 1000+  & 36.15 & 37.72 & 1000+ & 1000+ \\
FedAvg +FedMLB                           & \bf{49.36} & \bf{56.70}  & \bf{465} & \bf{602}  & \bf{39.34} & \bf{42.15} & \bf{441} & \bf{917} \\
\cline{1-9}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgM~\cite{hsu2019measuring}                & 46.66 & 52.49  & 572 &  937 & 38.41 & 40.75 & 475 & 1000+ \\
FedAvgM + FedMLB                                  & \bf{54.62} & \bf{60.91} & \bf{331} & \bf{417}  & \bf{43.96} & \bf{46.82} & \bf{294} & \bf{401} \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}                &50.81  &  56.95 & 427 & 569  & 40.13 & 42.75 & 415 & 813 \\
FedADAM + FedMLB                                  & \bf{53.34} & \bf{61.49}  & \bf{364} & \bf{467}  & \bf{40.67} & \bf{44.96} & 415 & \bf{610} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}                  &50.51  &56.79   & 427 & 580  & 39.39 & 42.97 & 423 & 875 \\
FedDyn + FedMLB                                  & \bf{57.51}  & \bf{62.43}   & \bf{298}  & \bf{355}  & \bf{43.35} & \bf{47.43} & \bf{294} & \bf{412} \\
\cline{1-9}
\end{tabular}}
\end{table*}






\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of federated learning methods on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_CIFAR_100}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 30.16& 38.11& 842& 1000+ \\
FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}                & 46.98  & 53.29  & 515 & 936  & 31.80 & 40.54 & 724 & 955  \\
FedAdam~\cite{reddi2021adaptive}                & 44.80  & 52.48  & 691 & 1000+  & 24.40 & 30.83 & 1000+ & 1000+  \\
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 293 & 504  & 33.52 & 45.01 & 576 & 714  \\
FedCM~\cite{xu2021fedcm}                            & 52.44  & 58.06  & 293 & 572  & 27.23 & 38.79 & 872 & 1000+ \\
FedAGM                                              & {57.04}  & {62.79}  & {245} & {353} & {35.68} & {48.40}  & {505} & {616}  \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {47.39} & {54.58} & {488} & {783} &{32.03} & {42.61}  & {642} & {800} \\
Ours + FedAGM                                              & \bf{61.32} & \bf{65.67} & \bf{216} & \bf{279} &\bf{41.10} & \bf{55.27}  & \bf{402} & \bf{479} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\begin{table*}[h]
\centering
\caption{Comparison of federated learning methods on Tiny-ImageNet with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_Tiny_ImageNet}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 35\% & 38\% & 500R           & \multicolumn{1}{c}{1000R}    & 24\%         & 30\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 33.94 & 35.42 & 645 &  1000+&23.63  & 29.48  & 523 &  1000+ \\
FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvgm~\cite{hsu2019measuring}                & 36.32 & 38.51 & 416 & 829 & 26.75 & 33.26  & 386 & 687  \\
FedAdam~\cite{reddi2021adaptive}                & 33.22 & 38.91 &  658& 945  & 21.88 & 28.08  & 648  & 1000+  \\
FedDyn~\cite{acar2020federated}                   & 38.86 & 42.82 & 327 & 440  & 27.74 & 37.25  & 387 & 580   \\
FedCM~\cite{xu2021fedcm}                            & 31.61 & 37.87 & 694 & 1000+ & 19.41 & 24.09  & 975 &  1000+ \\
FedAGM                                              & {42.26} & {46.31} & {226} & {331} &{31.47} & {38.48}  & {246} & {447} \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {37.20} & {40.16} & {414} & {539} &{28.39} & {33.67}  & {384} & {489} \\
Ours + FedAGM                                              & \bf{46.11} & \bf{50.54} & \bf{205} & \bf{260} &\bf{35.92} & \bf{43.85}  & \bf{209} & \bf{313} \\
\cline{1-9}
\end{tabular}}
\end{table*} 
\fi

==> ICML arxiv/tables/moreiteration.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Effect of more local iterations, $K = 100$ and $200$, for FedMLB and the baselines with other local objectives on CIFAR-100 with 100 clients and 5$\%$ participation rate. 
%\bhb{For the non-iid setting, we sample examples from a symmetric Dirichlet distribution parametrized by 0.3.}
The accuracy at the target round and the number of communication rounds to reach the target test accuracy are based on the exponential moving average with the momentum parameter $0.9$. 
%The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.
}
\label{tab:abl_local_iterations}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{$K = 100$ (Dir(0.3), 100 clients, 5\%)}                                                                     & \multicolumn{4}{c}{$K = 200$ (Dir(0.3), 100 clients, 5\%)}                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{Accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{Rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 48\% & 500R           & \multicolumn{1}{c}{1000R}    & 40\%         & 48\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.92  & 48.15  & 398 & 987  &41.45 &49.25 & 433& 897 \\
FedAvg + KD~\cite{hinton2014distilling}             & {42.58}  & {49.15}  & {385} & {905}   &42.84  & 51.48  & 381 & 751  \\
FedAvg + FitNet~\cite{romero2014fitnets}          &  39.48 & 45.80  & 531 & 1000+   & 37.17 & 43.97  & 651  & 1000+  \\%FedAvg + PodNet~\cite{douillard2020podnet}          &  41.98 & 48.18  & 396 & 993   & 41.29 & 48.92 &  459 &   910\\
%FedAvg + FitNets~\cite{}          &   &  &  &   &  &  &  &   \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.01  & 48.17  & 391 & 992 &  41.30& 48.67 & 458 &959\\
FedLS-NTD~\cite{lee2021preservation}                & 41.34 &  47.09 & 423 &  1000+ & 39.82 &46.72  & 508 & 1000+  \\
%MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{550} & \revision{875}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.04  & 46.79  & 387 & 1000+  & 42.26 & 48.85 &387 & 889 \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
FedMLB (ours)                                                & \bf{52.53} & \bf{58.52} & \bf{223} & \bf{359} & \bf{53.12} & \bf{58.91} & \bf{183} & \bf{325} \\
\cline{1-9}
\end{tabular}}
\end{table*}


==> ICML arxiv/tables/notation.tex <==
% !TEX root = ../main.tex

\begin{table}[h]
\centering
\caption{Summary of notation used in the paper}
\scalebox{0.9}{
\begin{tabular}{@{}cl@{}}
\hline
$N$ & total number of clients \\
$T$ & total number of communication rounds \\
$S_t$ & sampled number of clients in round $t$\\
$K$ & total number of local iterations \\
$i$ & client index \\
$D_i$ & data distribution of $i$th client \\
$\theta^t$ & shared model parameters in round $t$\\
%$\theta_{i}^t$ & local model of $i$th client in round $t$  \\
 $\theta_{i,k}^t$ & local model of $i$th client in round $t$ and step $k$  \\
 $M$ & total blocks of model \\
 $j$ & global branch index \\
 $y$ & labels of data \\
\hline
\end{tabular}}
\label{tab:notation}
\end{table}

==> ICML arxiv/tables/temp_analysis.tex <==
% !TEX root = ../main.tex
%
\begin{table}[t]
\centering
\caption{Sensitivity of FedMLB to $\tau^{\prime}$ with respect to the accuracy after 1$K$ rounds on CIFAR-100 in the moderate-scale setting with two different \iffalse Dirichlet parameters.\fi values of the symmetric Dirichlet parameter.}
\label{tab:temperature_sensitivity}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{ccccccc} 
%\cline{1-13}
$\tau^{\prime}$                & 0.75& 1 & 1.5 & 2 & 3 & 5 \\            
\cline{0-6}
Dir(0.3)                & 53.90& 54.58  &53.87 & 53.98 & 53.60 & 53.68  \\
Dir(0.6)                & 56.10 & 56.70 & 56.72 & 56.87 & 54.98 & 54.02 \\     
%IID                      & 57.26 & 56.40 & 56.68 & 54.95 & 54.82 & 54.07 \\     
\cline{0-6}
\end{tabular}}
%\vspace{-0.2cm}
\end{table}


\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> algorithms/fedavg.tex <==
% !TEX root = ../main.tex

\iffalse
\begin{algorithm}[t]
\caption{Federated learning framework}
\label{alg:fedavg}
\SetAlgoLined

\KwIn{$\theta^0$, number of clients $N$, number of local iterations $K$, number of communication rounds $T$}
\For{$\text{each round}~t = 0, \dots ,T$}{
Sample subset of clients $S_t \subseteq \{1, \dots, N\}$

Server sends $\theta^t$ to all clients $i \in S_t$ 

\For{$\text{each client}~ i \in S_t,~\textbf{in parallel}$}{
\For{$k = 0, \dots ,K$}{
{$\operatorname*{\underset{\theta_{i,k}^t}{argmin}}\ L_i(\theta_{i,k}^t
)$} ~~~ \dots \cref{fedavg_loss} and \cref{proposed_loss}
}
Client sends  $\theta_{i,K}^t$ back to the server}
\textbf{In server:}

\quad $\theta^{t+1}$ = $\frac{1}{|S_t|} \Sigma_{i \in S_t}\theta_{i,K}^{t}$
}
\textbf{Return} ~ $\theta^{t+1}$ 

\end{algorithm}
\fi

\begin{algorithm}[tb]
   \caption{FedAvg}
   \label{alg:fedavg}
\begin{algorithmic}
   \STATE {\bfseries Input:} {\# of clients $N$, \# of communication rounds $T$, \\ \quad\quad\quad \# of local iterations $K$, initial server model $\theta^0$}
   \FOR{$\text{each}~t = 0, \dots ,T-1$}
   \STATE Sample a subset of clients $S_t \subseteq \{1, \dots, N\}$.
   \STATE Server sends $\theta^t$ to each of the clients $i \in S_t$.
   \FOR{$\text{each client}~ i \in S_t,~\textbf{in parallel}$}
   \STATE \revision{Initialize client model $\theta_{i, 0} = \theta^t$.}
   \FOR{$k = 1, \dots ,K$}
   %\FOR{$\text{each batch } \textbf{b} = \{x,y\} \text{ of } D_i$ }
   \STATE \revision{$q_L \leftarrow \text{softmax} \left (\frac{F_L^M}{\tau} \right)$}
   \STATE \revision{$\mathcal{L}_L \leftarrow \text{CrossEntropy}(q_L, y)$}
   \STATE \revision{$\theta_{i,k}^t \leftarrow \theta_{i,k-1}^t - \eta \nabla \mathcal{L}_L $}
   %\ENDFOR
   %\STATE {\bfseries In server:} \\ \quad $\theta^{t+1}$ = $\frac{1}{|S_t|} \Sigma_{i \in S_t}\theta_{i,K}^{t}$
   \ENDFOR
   \STATE Client sends  $\theta_{i,K}^t$ back to the server.
   \ENDFOR
   \STATE {\bfseries In server:} \\ \quad $\theta^{t+1} = \frac{1}{|S_t|} \sum_{i \in S_t} \theta_{i,K}^{t}$
   \ENDFOR
\end{algorithmic}
\end{algorithm}


==> tables/Feddistill.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$, 100 clients}                                                                     & \multicolumn{4}{c}{2$\%$, 500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\% & 500R           & \multicolumn{1}{c}{1000R}    & 30\%         & 36\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.54  & 47.57  & 428 & 939  & 29.87& 37.48& 504& 858 \\
FedProx~\cite{li2020federated}                      & 42.03  & 47.93  & 419 & 886 & 29.28 & 36.16 & 533 & 966  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 386 &  740 & 28.66 &35.99  & 546 & 1000+  \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 397 & 872  & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
FedMLB                                                & \bf{47.39} & \bf{54.58} & \bf{339} & \bf{488} & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> tables/KD_FitNet.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparisons between FedMLB and the baselines with the standard knowledge distillation techniques on CIFAR-100. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_kd}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$, 100 clients}                                                                     & \multicolumn{4}{c}{2$\%$, 500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\% & 500R           & \multicolumn{1}{c}{1000R}    & 30\%         & 36\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.54  & 47.57  & 428 & 939  & 29.87& 37.48& 504& 858 \\
FedAvg + KD~\cite{hinton2014distilling}             & {42.99}  & {49.17}  & {389} & {752}   & {29.83} & {37.65}  & {505} & {859}  \\
FedAvg + FitNet~\cite{romero2014fitnets}          &  42.04 & 47.67  & 419 &914   & 29.92 &37.63  &503  & 860  \\
FedMLB                                                & \bf{47.39} & \bf{54.58} & \bf{339} & \bf{488} & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> tables/dummy.tex <==
% !TEX root = ../main.tex
%
\iffalse
\begin{table*}[h]
\centering
\caption{Comparison of federated learning methods on CIFAR-100: Dirichlet (0.6) split on 5\% client participation out of 100 clients. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:abl_dir06}
\scalebox{0.9}{
\begin{tabular}{lcccc} 
%\cline{1-13}
%& \multicolumn{8}{c}{Local epochs}  \\
%\cline{2-9}

\cline{2-5}
 \multirow{2}{*}{Methods} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 54\% & 58\%                \\ 
\cline{1-5}
FedAvg~\cite{mcmahan2017communication} & 43.91 & 49.18& 1000+ &1000+  \\
FedProx~\cite{li2020federated}                 & 43.15 &48.45 &1000+ &  1000+ \\
FedAvgm~\cite{hsu2019measuring}               &46.66  & 52.49 & 1000+ & 1000+  \\
FedAdam~\cite{reddi2021adaptive}              &45.95 & 51.63 & 1000+& 1000+ \\
FedDyn~\cite{acar2020federated}                  & 53.74 &59.70 & 518&   776   \\
FedCM~\cite{xu2021fedcm}                            &53.75 &60.48 & 511&    740   \\
FedAGM                                              &{58.82} &{63.88} & {325}&  {471} \\
Ours                                              &  {49.25} & {56.26}  & {757} & {1000+} \\
Ours + FedAGM                                              &  \bf{62.29} & \bf{66.79}  & \bf{276} & \bf{349} \\
\cline{1-5}
\end{tabular}}
\end{table*}

\begin{table*}[t]
\centering
\caption{Comparison of federated learning methods when the number of local iterations is 100 on CIFAR-100: Dirichlet (0.3) split on 5\% client participation out of 100 clients. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:abl_local_iterations}
\scalebox{0.9}{
\begin{tabular}{lcccc} 
%\cline{1-13}
%& \multicolumn{8}{c}{Local epochs}  \\
%\cline{2-9}
 Local iterations & \multicolumn{4}{c}{$K$ = 100}  \\ 
\cline{2-5}
 \multirow{2}{*}{Methods} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\%                \\ 
\cline{1-5}
FedAvg~\cite{mcmahan2017communication} &41.92 & 48.16  & 896 & 1000+  \\
FedProx~\cite{li2020federated}                 &  42.01 & 48.17  & 888 &  1000+ \\
FedAvgm~\cite{hsu2019measuring}               &  45.72 &  52.74 & 578 & 1000+  \\
FedAdam~\cite{reddi2021adaptive}              &  43.00 &  47.51 & 994  &  1000+ \\
FedDyn~\cite{acar2020federated}                  &  51.98 & 59.13  &347  & 532   \\
FedCM~\cite{xu2021fedcm}                            &  46.90 & 54.20  & 502 & 893  \\
FedAGM                                              &  {54.71} & {63.12}  & {284} & {461} \\
Ours                                              &  {52.53} & {58.52}  & {341} & {525} \\
Ours + FedAGM                                              &  \bf{57.62} & \bf{65.89}  & \bf{238} & \bf{357} \\
\cline{1-5}
\end{tabular}}
\end{table*}
\fi


==> tables/lambdaCE_analysis.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{$\mathcal{L}_{G}^\text{CE}$ analysis}
\label{tab:local_approaches}
\scalebox{0.9}{
\begin{tabular}{ccccc} 
%\cline{1-13}
\multirow{3}{*}{$\mathcal{L}_{G}^\text{CE}$}                                   & \multicolumn{3}{c}{5$\%$,100 clients}   \\                                                                                                                                                                                                                
\cline{2-5}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}   \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\%  \\ 
\cline{1-5}
0.75                & 29.87& 37.48& 504& 858 \\
1                & {29.83} & {37.65}  & {505} & {859}  \\
1.25            & 28.89 &36.11  &551  & 995  \\
1.5                      & 29.28 & 36.16 & 533 & 966  \\
2                 & 28.66 &35.99  & 546 & 1000+  \\
3                              & \revision{38.36}  & \revision{48.61}  & \revision{550} & \revision{875}    \\
5                            & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
10                                                 & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-5}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> tables/lambdaKL_analysis.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{$\mathcal{L}_{G}^{\text{KL}}$ analysis}
\label{tab:local_approaches}
\scalebox{0.9}{
\begin{tabular}{ccccc} 
%\cline{1-13}
\multirow{3}{*}{$\mathcal{L}_{G}^{\text{KL}}$}                                   & \multicolumn{3}{c}{5$\%$,100 clients}   \\                                                                                                                                                                                                                
\cline{2-5}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}   \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\%  \\ 
\cline{1-5}
0.75                & 29.87& 37.48& 504& 858 \\
1                & {29.83} & {37.65}  & {505} & {859}  \\
1.25            & 28.89 &36.11  &551  & 995  \\
1.5                      & 29.28 & 36.16 & 533 & 966  \\
2                 & 28.66 &35.99  & 546 & 1000+  \\
3                              & \revision{38.36}  & \revision{48.61}  & \revision{550} & \revision{875}    \\
5                            & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
10                                                 & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-5}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> tables/large_clients.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a large number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 500, 2\%, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:large_clients}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 36\% & 40\% & 500R           & \multicolumn{1}{c}{1000R}    & 26\%         & 32\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 29.87& 37.48& 858& 1000+ &23.63  & 29.48  & 645 &  1000+ \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvg + FedMLB                           & \bf{32.03} & \bf{42.61}  & \bf{642} & \bf{800} &{\bf28.39} & {\bf33.67}  & {\bf429} & {\bf710} \\
\cline{1-9}
FedAvgm~\cite{hsu2019measuring}                & 31.80 & 40.54 & 724 & 955 & 26.75 & 33.26  & 457 & 836  \\
FedAvgm + FedMLB                           & \bf{36.21} & \bf{47.75}  & \bf{496} & \bf{636} &{\bf32.00} & {\bf37.53}  & {\bf307} & {\bf500} \\
\cline{1-9}
FedAdam~\cite{reddi2021adaptive}                & 36.07 & 47.04 & 480 & 653  & 29.65 & 35.91  & 345  & 642  \\
FedAdam + FedMLB                          & \bf{38.28} & \bf{52.68}  & \bf{442} & \bf{527} &{\bf32.14} & {\bf39.54}  & {\bf311} & {\bf524} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}                   & 31.58 & 41.02 & 691 & 927  &24.35 & 29.54  & 595 & 1000+   \\
FedDyn + FedMLB                           & \bf{36.50} & \bf{49.65}  & \bf{478} & \bf{611} &{\bf30.77} & {\bf37.68}  & {\bf384} & {\bf541} \\
\cline{1-9}
\end{tabular}}
\end{table*}

==> tables/large_clients_IID.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a large number of clients with IID distribution. In these experiments, the number of clients and participation rate are set to 500 and 2\%, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:large_clients_IID}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 36\% & 44\% & 500R           & \multicolumn{1}{c}{1000R}    & 26\%         & 32\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  &{29.96}& {36.93}& {903}  & {1000+} & 23.25  & 28.92 & 701 & 1000+   \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvg + FedMLB                           & \bf{34.60} &\bf{ 44.95}  & \bf{549} & \bf{ 935} & \bf{28.27} &\bf{ 35.51} &\bf{ 435} &\bf{ 689} \\
\cline{1-9}
FedAvgM~\cite{hsu2019measuring}         & 32.47 & 41.04  & 679 &  1000+ & 27.52 & 34.08 & 445 & 800 \\
FedAvgM + FedMLB                          &\bf{ 38.60} &\bf{50.52}   & \bf{418} & \bf{676}  & \bf{33.51} &  & \bf{281} &\bf{444}  \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}        &38.32  &  48.70 & 430 & 712  &  &  & 252 & 441 \\
FedADAM + FedMLB                          &\bf{42.48} &  \bf{55.24} &\bf{338}  &\bf{539 }  &  &  & \bf{250} & \bf{384 }\\
\cline{1-9}
FedDyn~\cite{acar2020federated}         &  35.77& 47.34  & 509 &  806 & 24.79 &  &565  &  \\
FedDyn + FedMLB                           & \bf{39.37} & \bf{53.11}  & \bf{429} & \bf{619}  & \bf{30.46} & \bf{37.89 }& \bf{384} & \bf{540} \\
\cline{1-9}
\end{tabular}}
\end{table*}

==> tables/large_clients_dir06.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a large number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 500, 2\%, and $0.6$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:large_clients_dir06}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 29.36 &  36.36 &  966& 1000+  & 24.48 & 29.94 & 600 & 1000+ \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvg + FedMLB                           &\bf{33.74}  & \bf{43.53}  & \bf{571} & 1000+  & \bf{28.97} & \bf{35.08} & \bf{415} & \bf{650} \\
\cline{1-9}
FedAvgM~\cite{hsu2019measuring}         & 32.44 & 41.40  & 680 & 1000+  & 24.65 & 31.54 & 575 & 1000+ \\
FedAvgM + FedMLB                          & \bf{38.35} & \bf{49.65} & \bf{421} & \bf{690}  & \bf{32.33} & \bf{37.6} & \bf{308} & \bf{483} \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}        & 37.33 &  47.73 & 463 &756   & 31.4 & 37.03 & \bf{286} & 876 \\
FedADAM + FedMLB                           &\bf{39.57}  & \bf{53.53}  & \bf{402} & \bf{621}  & \bf{33.71} & \bf{41.15} & 292 & \bf{619} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}         & 31.63 & 41.58  & 677 & 1000+  & 26.42 & 31.80 & 485 & 1000+ \\
FedDyn + FedMLB                          & \bf{38.90} & \bf{52.72}  & \bf{440} & \bf{639}  & \bf{32.52} & \bf{38.28} & \bf{350} & \bf{712} \\\cline{1-9}
\end{tabular}}
\end{table*}

==> tables/local_approaches_IID.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\% & 500R           & \multicolumn{1}{c}{1000R}    & 30\%         & 36\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 924  & 29.87& 37.48& 504& 858 \\
FedAvg + KD~\cite{hinton2014distilling}             & {42.99}  & {49.17}  & {389} & {752}   & {29.83} & {37.65}  & {505} & {859}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 434 &1000+   & 28.89 &36.11  &551  & 995  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 425 & 881 & 29.28 & 36.16 & 533 & 966  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 386 &  740 & 28.66 &35.99  & 546 & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{550} & \revision{875}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 397 & 872  & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{339} & \bf{488} & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> tables/local_approaches_dir06.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 40\% & 47\% & 500R           & \multicolumn{1}{c}{1000R}    & 30\%         & 36\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 924  & 29.87& 37.48& 504& 858 \\
FedAvg + KD~\cite{hinton2014distilling}             & {42.99}  & {49.17}  & {389} & {752}   & {29.83} & {37.65}  & {505} & {859}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 434 &1000+   & 28.89 &36.11  &551  & 995  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 425 & 881 & 29.28 & 36.16 & 533 & 966  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 386 &  740 & 28.66 &35.99  & 546 & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{550} & \revision{875}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 397 & 872  & 29.27 & 37.25 & 530&896  \\
%LFGN                          & 44.90  & 51.05  & 342 & 623  & 32.40 & 39.44 & \bf{408}&695  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{339} & \bf{488} & \bf{32.03} & \bf{42.61} & \bf{446} & \bf{642} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines which revise local objective functions on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:local_approaches}
\scalebox{1.0}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%  \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}              & 41.88  & 47.83  & 924 & 1000+  & 29.87& 37.48& 858& 1000+ \\
FedAvg + KD~\cite{hinton2014distilling}             & \revision{41.23}  & \revision{47.34}  & \revision{940} & \revision{1000+}   & \revision{29.42} & \revision{37.11}  & \revision{909} & \revision{1000+}  \\
FedAvg + PodNet~\cite{douillard2020podnet}          &  41.22 & 46.86  & 1000+ &1000+   & 28.89 &36.11  &995  & 1000+  \\
\cdashline{1-9}
FedProx~\cite{li2020federated}                      & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedLS-NTD~\cite{lee2021preservation}                & 43.22 &  49.29 & 740 &  1000+ & 28.66 &35.99  & 1000+ & 1000+  \\
MOON\cite{li2021model}                              & \revision{38.36}  & \revision{48.61}  & \revision{875} & \revision{1000+}  &  &  &  &   \\
FedGKD~\cite{yao2021local}                          & 42.28  & 47.96  & 872 & 1000+  & 29.27 & 37.25 & 896&1000+  \\
Ours                                                & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} & \bf{32.03} & \bf{42.61} & \bf{642} & \bf{800} \\
\cline{1-9}
\end{tabular}}
\end{table*}
\fi

==> tables/low_participation.tex <==
% !TEX root = ../main.tex
%
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-10 and CIFAR-100 with low participation rates (1\%). In these experiments, the number of clients and Dirichlet parameter are set to 100, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10} & \multicolumn{4}{c}{CIFAR-100} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 46.72 & 64.33 &  &   &  &  &  &  \\
FedAvg + Ours                           & 37.45 & 57.24 &  &  & &  &  &  \\
\cline{1-9}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}         & 46.05 & 63.73  &  &   &  &  &  &   \\
FedAvgm + Ours                          & 41.41 & 43.25  &  &   &  &  &  & \\
\cline{1-9}
FedAdam~\cite{reddi2021adaptive}        & 37.42 & 51.94  &  &  &  &  &  &   \\
FedAdam + Ours                          & 19.76 & 23.78 &  &  &  &  &  &  \\
\cline{1-9}
FedDyn~\cite{acar2020federated}         & 50.60 & 68.72 &  &   &  &  &  &   \\
FedDyn + Ours                           & 41.41 & 64.54  &  &   &  &  &  &  \\
\cline{1-9}
\end{tabular}}
\end{table*}



==> tables/moderate_clients.tex <==
% !TEX root = ../main.tex
%
\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR10, CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients}
\scalebox{0.9}{
\begin{tabular}{lcccccccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-13}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-13}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 33.94 & 35.42 & 645 &  1000+ \\
FedAvg + Ours                                              & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} &{\bf37.20} & {\bf40.16} & {\bf414} & {\bf539} \\
\cline{1-13}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgM~\cite{hsu2019measuring}                & 46.98  & 53.24  & 515 & 936  & 36.10 & 38.36  & 794& 1000+  \\
FedAvgm + Ours                                             & \bf{53.02} & \bf{58.97} & \bf{349} & \bf{499} & {\bf40.93} & {\bf43.52} & {\bf309} & {\bf380} \\
\cline{1-13}
FedAdam~\cite{reddi2021adaptive}                & 44.80  & \bf{52.48}  & 691 & 1000+  & 33.22 & 38.91 &  658& 945  \\
FedAdam + Ours                                              & \bf{46.04} & {51.12} & \bf{653} & {1000+} & {\bf33.49} & {\bf38.93} & {\bf640} & {\bf785} \\
\cline{1-13}
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 317 & 521  & 38.86 & 42.82 & 327 & 440  \\
FedDyn + Ours                                              & \bf{57.33} & \bf{61.81} & \bf{299} & \bf{377} &{\bf43.05} & {\bf46.55} & {\bf283} & {\bf324} \\
\cline{1-13}
\end{tabular}}
\end{table*}
\fi


\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is marked in {\bf bold}.}
\label{tab:moderate_clients}
\vspace{0.1cm}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 38\%         & 42\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 33.94 & 35.42  &  1000+& 1000+ \\
FedAvg + FedMLB                                              & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} &{\bf37.20} & {\bf40.16}  & {\bf539}& {1000+} \\
\cline{1-9}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgM~\cite{hsu2019measuring}                & 46.98  & 53.24  & 515 & 936  & 36.10 & 38.36  & 794& 1000+  \\
FedAvgm + FedMLB                                             & \bf{53.02} & \bf{58.97} & \bf{349} & \bf{499} & {\bf40.93} & {\bf43.52} & {\bf380}& {\bf642}  \\
\cline{1-9}
FedAdam~\cite{reddi2021adaptive}                & 47.07  & {54.19}  & 499 & 947  & \bf{36.98} & 40.6 & 647 &  1000+ \\
FedAdam + FedMLB                                              & \bf{48.59} & \bf{58.23} & \bf{472} &\bf{645} & {35.81} & {\bf42.9}  & {\bf552}& {\bf873} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}                  & 48.38  & 55.78  & 425 & 735
&37.35&41.17&573&1000+ \\
FedDyn + FedMLB                                              & \bf{57.33} & \bf{61.81} & \bf{299} & \bf{377} &{\bf43.05} & {\bf46.55}  & {\bf324}& {\bf446} \\
\cline{1-9}\end{tabular}}
\end{table*}






\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of federated learning methods on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_CIFAR_100}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 30.16& 38.11& 842& 1000+ \\
FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}                & 46.98  & 53.29  & 515 & 936  & 31.80 & 40.54 & 724 & 955  \\
FedAdam~\cite{reddi2021adaptive}                & 44.80  & 52.48  & 691 & 1000+  & 24.40 & 30.83 & 1000+ & 1000+  \\
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 293 & 504  & 33.52 & 45.01 & 576 & 714  \\
FedCM~\cite{xu2021fedcm}                            & 52.44  & 58.06  & 293 & 572  & 27.23 & 38.79 & 872 & 1000+ \\
FedAGM                                              & {57.04}  & {62.79}  & {245} & {353} & {35.68} & {48.40}  & {505} & {616}  \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {47.39} & {54.58} & {488} & {783} &{32.03} & {42.61}  & {642} & {800} \\
Ours + FedAGM                                              & \bf{61.32} & \bf{65.67} & \bf{216} & \bf{279} &\bf{41.10} & \bf{55.27}  & \bf{402} & \bf{479} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\begin{table*}[h]
\centering
\caption{Comparison of federated learning methods on Tiny-ImageNet with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_Tiny_ImageNet}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 35\% & 38\% & 500R           & \multicolumn{1}{c}{1000R}    & 24\%         & 30\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 33.94 & 35.42 & 645 &  1000+&23.63  & 29.48  & 523 &  1000+ \\
FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvgm~\cite{hsu2019measuring}                & 36.32 & 38.51 & 416 & 829 & 26.75 & 33.26  & 386 & 687  \\
FedAdam~\cite{reddi2021adaptive}                & 33.22 & 38.91 &  658& 945  & 21.88 & 28.08  & 648  & 1000+  \\
FedDyn~\cite{acar2020federated}                   & 38.86 & 42.82 & 327 & 440  & 27.74 & 37.25  & 387 & 580   \\
FedCM~\cite{xu2021fedcm}                            & 31.61 & 37.87 & 694 & 1000+ & 19.41 & 24.09  & 975 &  1000+ \\
FedAGM                                              & {42.26} & {46.31} & {226} & {331} &{31.47} & {38.48}  & {246} & {447} \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {37.20} & {40.16} & {414} & {539} &{28.39} & {33.67}  & {384} & {489} \\
Ours + FedAGM                                              & \bf{46.11} & \bf{50.54} & \bf{205} & \bf{260} &\bf{35.92} & \bf{43.85}  & \bf{209} & \bf{313} \\
\cline{1-9}
\end{tabular}}
\end{table*} 
\fi

==> tables/moderate_clients_IID.tex <==
% !TEX root = ../main.tex
%
\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR10, CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients}
\scalebox{0.9}{
\begin{tabular}{lcccccccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-13}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-13}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 33.94 & 35.42 & 645 &  1000+ \\
FedAvg + Ours                                              & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} &{\bf37.20} & {\bf40.16} & {\bf414} & {\bf539} \\
\cline{1-13}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}                & 46.98  & 53.29  & 515 & 936  & 36.32 & 38.51 & 416 & 829  \\
FedAvgm + Ours                                             & \bf{53.02} & \bf{58.97} & \bf{349} & \bf{499} & {\bf40.93} & {\bf43.52} & {\bf309} & {\bf380} \\
\cline{1-13}
FedAdam~\cite{reddi2021adaptive}                & 44.80  & \bf{52.48}  & 691 & 1000+  & 33.22 & 38.91 &  658& 945  \\
FedAdam + Ours                                              & \bf{46.04} & {51.12} & \bf{653} & {1000+} & {\bf33.49} & {\bf38.93} & {\bf640} & {\bf785} \\
\cline{1-13}
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 317 & 521  & 38.86 & 42.82 & 327 & 440  \\
FedDyn + Ours                                              & \bf{57.33} & \bf{61.81} & \bf{299} & \bf{377} &{\bf43.05} & {\bf46.55} & {\bf283} & {\bf324} \\
\cline{1-13}
\end{tabular}}
\end{table*}
\fi


\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients and participation rate are set to 100 and 5\% with IID distribution. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients_IID}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 48\% & 52\% & 500R           & \multicolumn{1}{c}{1000R}    & 38\%         & 42\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 43.60 &  48.01 &  997& 1000+  & 37.96 & 38.92 & 504 & 1000+ \\
%FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvg + FedMLB                           &\bf{50.12}  &\bf{ 56.40  }&\bf{ 426} &\bf{ 584  }& \bf{40.69} & \bf{42.98} & \bf{376} & \bf{640} \\
\cline{1-9}
FedAvgM~\cite{hsu2019measuring}         & 47.43 & 52.83  & 532 & 880  & 39.79 & 41.34 & 346 & 1000+ \\
FedAvgM + FedMLB                          & \bf{55.29} & \bf{61.16}  & \bf{294} & \bf{377  }& \bf{44.02} & \bf{47.03} & \bf{271 }& \bf{382} \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}        & 54.35 &  60.35 & 303 &416   & 43.54 &  46.12& \bf{257} & 377 \\
FedADAM + FedMLB                           &\bf{57.13}  & \bf{62.58}  & \bf{285} & \bf{363 } & \bf{44.27} &\bf{ 47.36} &276  &\bf{ 372} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}         & 50.37 & 56.88  & 397 & 592  & 39.49 &  42.42& 350 & 848 \\
FedDyn + FedMLB                           & \bf{56.97 }& \bf{61.41}  & \bf{298} & \bf{366}  & \bf{44.28} &  & \bf{277} & \bf{361} \\
\cline{1-9}\end{tabular}}
\end{table*}





\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of federated learning methods on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_CIFAR_100}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 30.16& 38.11& 842& 1000+ \\
FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}                & 46.98  & 53.29  & 515 & 936  & 31.80 & 40.54 & 724 & 955  \\
FedAdam~\cite{reddi2021adaptive}                & 44.80  & 52.48  & 691 & 1000+  & 24.40 & 30.83 & 1000+ & 1000+  \\
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 293 & 504  & 33.52 & 45.01 & 576 & 714  \\
FedCM~\cite{xu2021fedcm}                            & 52.44  & 58.06  & 293 & 572  & 27.23 & 38.79 & 872 & 1000+ \\
FedAGM                                              & {57.04}  & {62.79}  & {245} & {353} & {35.68} & {48.40}  & {505} & {616}  \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {47.39} & {54.58} & {488} & {783} &{32.03} & {42.61}  & {642} & {800} \\
Ours + FedAGM                                              & \bf{61.32} & \bf{65.67} & \bf{216} & \bf{279} &\bf{41.10} & \bf{55.27}  & \bf{402} & \bf{479} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\begin{table*}[h]
\centering
\caption{Comparison of federated learning methods on Tiny-ImageNet with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_Tiny_ImageNet}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 35\% & 38\% & 500R           & \multicolumn{1}{c}{1000R}    & 24\%         & 30\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 33.94 & 35.42 & 645 &  1000+&23.63  & 29.48  & 523 &  1000+ \\
FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvgm~\cite{hsu2019measuring}                & 36.32 & 38.51 & 416 & 829 & 26.75 & 33.26  & 386 & 687  \\
FedAdam~\cite{reddi2021adaptive}                & 33.22 & 38.91 &  658& 945  & 21.88 & 28.08  & 648  & 1000+  \\
FedDyn~\cite{acar2020federated}                   & 38.86 & 42.82 & 327 & 440  & 27.74 & 37.25  & 387 & 580   \\
FedCM~\cite{xu2021fedcm}                            & 31.61 & 37.87 & 694 & 1000+ & 19.41 & 24.09  & 975 &  1000+ \\
FedAGM                                              & {42.26} & {46.31} & {226} & {331} &{31.47} & {38.48}  & {246} & {447} \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {37.20} & {40.16} & {414} & {539} &{28.39} & {33.67}  & {384} & {489} \\
Ours + FedAGM                                              & \bf{46.11} & \bf{50.54} & \bf{205} & \bf{260} &\bf{35.92} & \bf{43.85}  & \bf{209} & \bf{313} \\
\cline{1-9}
\end{tabular}}
\end{table*} 
\fi

==> tables/moderate_clients_dir06.tex <==
% !TEX root = ../main.tex
%
\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR10, CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and $0.3$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients}
\scalebox{0.9}{
\begin{tabular}{lcccccccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-13}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-13}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 33.94 & 35.42 & 645 &  1000+ \\
FedAvg + Ours                                              & \bf{47.39} & \bf{54.58} & \bf{488} & \bf{783} &{\bf37.20} & {\bf40.16} & {\bf414} & {\bf539} \\
\cline{1-13}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}                & 46.98  & 53.29  & 515 & 936  & 36.32 & 38.51 & 416 & 829  \\
FedAvgm + Ours                                             & \bf{53.02} & \bf{58.97} & \bf{349} & \bf{499} & {\bf40.93} & {\bf43.52} & {\bf309} & {\bf380} \\
\cline{1-13}
FedAdam~\cite{reddi2021adaptive}                & 44.80  & \bf{52.48}  & 691 & 1000+  & 33.22 & 38.91 &  658& 945  \\
FedAdam + Ours                                              & \bf{46.04} & {51.12} & \bf{653} & {1000+} & {\bf33.49} & {\bf38.93} & {\bf640} & {\bf785} \\
\cline{1-13}
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 317 & 521  & 38.86 & 42.82 & 327 & 440  \\
FedDyn + Ours                                              & \bf{57.33} & \bf{61.81} & \bf{299} & \bf{377} &{\bf43.05} & {\bf46.55} & {\bf283} & {\bf324} \\
\cline{1-13}
\end{tabular}}
\end{table*}
\fi


\begin{table*}[t]
\centering
\caption{Comparison of the proposed method with baselines on CIFAR-100 and Tiny-ImageNet with a moderate number of clients. In these experiments, the number of clients, participation rate, and Dirichlet parameter are set to 100, 5\%, and $0.6$, respectively. Accuracy at target round and the communication round to reach target test accuracy is based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted in {\bf bold}.}
\label{tab:moderate_clients_dir06}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{Tiny-ImageNet} \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 48\% & 52\% & 500R           & \multicolumn{1}{c}{1000R}    & 38\%         & 42\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 43.43 & 48.71  & 926 & 1000+  & 36.15 & 37.72 & 1000+ & 1000+ \\
FedAvg +FedMLB                           & \bf{49.36} & \bf{56.70}  & \bf{465} & \bf{602}  & \bf{39.34} & \bf{42.15} & \bf{441} & \bf{917} \\
\cline{1-9}
%FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgM~\cite{hsu2019measuring}                & 46.66 & 52.49  & 572 &  937 & 38.41 & 40.75 & 475 & 1000+ \\
FedAvgM + FedMLB                                  & \bf{54.62} & \bf{60.91} & \bf{331} & \bf{417}  & \bf{43.96} & \bf{46.82} & \bf{294} & \bf{401} \\
\cline{1-9}
FedADAM~\cite{reddi2021adaptive}                &50.81  &  56.95 & 427 & 569  & 40.13 & 42.75 & 415 & 813 \\
FedADAM + FedMLB                                  & \bf{53.34} & \bf{61.49}  & \bf{364} & \bf{467}  & \bf{40.67} & \bf{44.96} & 415 & \bf{610} \\
\cline{1-9}
FedDyn~\cite{acar2020federated}                  &50.51  &56.79   & 427 & 580  & 39.39 & 42.97 & 423 & 875 \\
FedDyn + FedMLB                                  & \bf{57.51}  & \bf{62.43}   & \bf{298}  & \bf{355}  & \bf{43.35} & \bf{47.43} & \bf{294} & \bf{412} \\
\cline{1-9}
\end{tabular}}
\end{table*}






\iffalse
\begin{table*}[t]
\centering
\caption{Comparison of federated learning methods on CIFAR-100 with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_CIFAR_100}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 47\% & 53\% & 500R           & \multicolumn{1}{c}{1000R}    & 36\%         & 40\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 41.88  & 47.83  & 924 & 1000+  & 30.16& 38.11& 842& 1000+ \\
FedProx~\cite{li2018federated}                        & 42.43  & 48.32  & 881 & 1000+ & 29.28 & 36.16 & 966 & 1000+  \\
FedAvgm~\cite{hsu2019measuring}                & 46.98  & 53.29  & 515 & 936  & 31.80 & 40.54 & 724 & 955  \\
FedAdam~\cite{reddi2021adaptive}                & 44.80  & 52.48  & 691 & 1000+  & 24.40 & 30.83 & 1000+ & 1000+  \\
FedDyn~\cite{acar2020federated}                  & 52.66  & 58.46  & 293 & 504  & 33.52 & 45.01 & 576 & 714  \\
FedCM~\cite{xu2021fedcm}                            & 52.44  & 58.06  & 293 & 572  & 27.23 & 38.79 & 872 & 1000+ \\
FedAGM                                              & {57.04}  & {62.79}  & {245} & {353} & {35.68} & {48.40}  & {505} & {616}  \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {47.39} & {54.58} & {488} & {783} &{32.03} & {42.61}  & {642} & {800} \\
Ours + FedAGM                                              & \bf{61.32} & \bf{65.67} & \bf{216} & \bf{279} &\bf{41.10} & \bf{55.27}  & \bf{402} & \bf{479} \\
\cline{1-9}
\end{tabular}}
\end{table*}



\begin{table*}[h]
\centering
\caption{Comparison of federated learning methods on Tiny-ImageNet with two different settings. Accuracy at the target round and the communication round to reach target test accuracy are based on running exponential moving average with parameter $0.9$. The arrows indicate whether higher ($\uparrow$) or lower ($\downarrow$) is better. The best performance in each column is denoted by {\bf bold}.}
\label{tab:abl_Tiny_ImageNet}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
%\cline{1-13}
\multirow{3}{*}{Method}                                   & \multicolumn{4}{c}{5$\%$,100 clients}                                                                     & \multicolumn{4}{c}{2$\%$,500 clients }                                                                                                                                                                \\ 
\cline{2-9}
 & \multicolumn{2}{c}{accuracy (\%, $\uparrow$ )} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)} & \multicolumn{2}{c}{accuracy (\%, $\uparrow$)} & \multicolumn{2}{c}{rounds (\#, $\downarrow$)}  \\
& \multicolumn{1}{c}{500R} & \multicolumn{1}{c}{1000R} & 35\% & 38\% & 500R           & \multicolumn{1}{c}{1000R}    & 24\%         & 30\%                 \\ 
\cline{1-9}
FedAvg~\cite{mcmahan2017communication}  & 33.94 & 35.42 & 645 &  1000+&23.63  & 29.48  & 523 &  1000+ \\
FedProx~\cite{li2018federated}                        & 34.14 & 35.53 & 613 & 1000+ &25.45 & 31.71 & 445  & 799  \\
FedAvgm~\cite{hsu2019measuring}                & 36.32 & 38.51 & 416 & 829 & 26.75 & 33.26  & 386 & 687  \\
FedAdam~\cite{reddi2021adaptive}                & 33.22 & 38.91 &  658& 945  & 21.88 & 28.08  & 648  & 1000+  \\
FedDyn~\cite{acar2020federated}                   & 38.86 & 42.82 & 327 & 440  & 27.74 & 37.25  & 387 & 580   \\
FedCM~\cite{xu2021fedcm}                            & 31.61 & 37.87 & 694 & 1000+ & 19.41 & 24.09  & 975 &  1000+ \\
FedAGM                                              & {42.26} & {46.31} & {226} & {331} &{31.47} & {38.48}  & {246} & {447} \\ %\bf{30.86} & \bf{38.08}  & \bf{252} & \bf{447} \\
Ours                                              & {37.20} & {40.16} & {414} & {539} &{28.39} & {33.67}  & {384} & {489} \\
Ours + FedAGM                                              & \bf{46.11} & \bf{50.54} & \bf{205} & \bf{260} &\bf{35.92} & \bf{43.85}  & \bf{209} & \bf{313} \\
\cline{1-9}
\end{tabular}}
\end{table*} 
\fi

==> tables/notation.tex <==
% !TEX root = ../main.tex

\begin{table}[h]
\centering
\caption{Summary of notation used in the paper}
\scalebox{0.9}{
\begin{tabular}{@{}cl@{}}
\hline
$N$ & total number of clients \\
$T$ & total number of communication rounds \\
$S_t$ & sampled number of clients in round $t$\\
$K$ & total number of local iterations \\
$i$ & client index \\
$D_i$ & data distribution of $i$th client \\
$\theta^t$ & shared model parameters in round $t$\\
%$\theta_{i}^t$ & local model of $i$th client in round $t$  \\
 $\theta_{i,k}^t$ & local model of $i$th client in round $t$ and step $k$  \\
 $M$ & total blocks of model \\
 $j$ & global branch index \\
 $y$ & labels of data \\
\hline
\end{tabular}}
\label{tab:notation}
\end{table}
